Causal Effect Identification in Cluster DAGs

Reasoning about the effect of interventions and counterfactuals is a fundamental task found throughout the data sciences. A collection of principles, algorithms, and tools has been developed for performing such tasks in the last decades (Pearl, 2000). One of the pervasive requirements found throughout this literature is the articulation of assumptions, which commonly appear in the form of causal diagrams. Despite the power of this approach, there are significant settings where the knowledge necessary to specify a causal diagram over all variables is not available, particularly in complex, high-dimensional domains. In this paper, we introduce a new graphical modeling tool called cluster DAGs (for short, C-DAGs) that allows for the partial specification of relationships among variables based on limited prior knowledge, alleviating the stringent requirement of specifying a full causal diagram. A C-DAG specifies relationships between clusters of variables, while the relationships between the variables within a cluster are left unspecified, and can be seen as a graphical representation of an equivalence class of causal diagrams that share the relationships among the clusters. We develop the foundations and machinery for valid inferences over C-DAGs about the clusters of variables at each layer of Pearl's Causal Hierarchy (Pearl and Mackenzie 2018; Bareinboim et al. 2020) - L1 (probabilistic), L2 (interventional), and L3 (counterfactual). In particular, we prove the soundness and completeness of d-separation for probabilistic inference in C-DAGs. Further, we demonstrate the validity of Pearl's do-calculus rules over C-DAGs and show that the standard ID identification algorithm is sound and complete to systematically compute causal effects from observational data given a C-DAG. Finally, we show that C-DAGs are valid for performing counterfactual inferences about clusters of variables.

==> R-77-CDAGS - AAAI-2023/figs/1_ignorability.tex <==
\begin{figure}[t]
%\begin{wrapfigure}{r}{0.505\textwidth}
\vspace{-0.8\intextsep}
\begin{minipage}[t]{.32\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering	
\begin{tikzpicture}[scale = .6]
			\node(X) at (0,0) [label = below:X, point, blue];
			\node(Y) at (2, 0)[label = below:Y, point, red];
			\node[state](Z) at (1, 2) {$\*Z$}; 
			\path (X) edge (Y);
			\path (Z) edge (X);
			\path (Z) edge (Y);
		\end{tikzpicture} 
		\caption*{$G_{\*C_1}$}
		\vspace{1em}
\end{subfigure}
\end{minipage}
\begin{minipage}[t]{.32\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering	
    \begin{tikzpicture}[scale = .6]
			\node(X) at (0,0) [label = below:X, point, blue];
			\node(Y) at (2, 0)[label = below:Y, point, red];
			\node(Z1) at (0, 2)[label=left:{$Z_1$}, point]; 
			\node(Z2) at (2, 2)[label=right:{$Z_2$}, point];
			\path (X) edge (Y);
			\path (Z1) edge (X);
			\path (Z1) edge (Y);
			\path (Z2) edge (Y);
			\path (Z2) edge (X);
			\draw[gray, fill=gray!30, opacity =.5] (-.1,1.7) rectangle (2.1, 2.3);
		\end{tikzpicture} 
		\caption*{$(a)$}
		\vspace{0.7em}
\end{subfigure}
\end{minipage}
% \begin{minipage}[t]{.32\linewidth}
% \begin{subfigure}[b]{\linewidth}
% \centering	
%     \begin{tikzpicture}[scale = .6]
% 			\node(X) at (0,0) [label = below:X, point, blue];
% 			\node(Y) at (2, 0)[label = below:Y, point, red];
% 			\node(Z1) at (0, 2)[label=left:{$Z_1$}, point]; 
% 			\node(Z2) at (2, 2)[label=right:{$Z_2$}, point];
% 			\path (X) edge (Y);
% 			\path (Z1) edge (X);
% 			\path (Z2) edge (Y);
% 			\draw[gray, fill=gray!30, opacity =.5] (-.1,1.7) rectangle (2.1, 2.3);
% 		\end{tikzpicture} 
% 		\caption*{$(b): Y_x \indep X \mid \*Z$}
% \end{subfigure}
% \end{minipage}
\begin{minipage}[t]{.32\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering	
\begin{tikzpicture}[scale = .6]
			\node(X) at (0,0) [label = below:X, point, blue];
			\node(Y) at (2, 0)[label = below:Y, point, red];
			\node(Z1) at (0, 2)[label=left:{$Z_1$}, point]; 
			\node(Z2) at (2, 2)[label=right:{$Z_2$}, point];
			\path (X) edge (Y);
			\path (Z1) edge (X);
			\path (Z1) edge (Y);
			\path (Z2) edge (Y);
			\path (Z2) edge (X);
			\path[bidirected] (Z1) edge[bend left =10] (Z2);
			\draw[gray, fill=gray!30, opacity =.5] (-.1,1.7) rectangle (2.1, 2.3);
		\end{tikzpicture} 
		\caption*{$(b)$}
		\vspace{0.7em}
\end{subfigure}
\end{minipage}	
% \begin{minipage}[t]{.32\linewidth}
% \begin{subfigure}[b]{\linewidth}
% \centering	
% \begin{tikzpicture}[scale = .6]
% 			\node(X) at (0,0) [label = below:X, point, blue];
% 			\node(Y) at (2, 0)[label = below:Y, point, red];
% 			\node(Z1) at (0, 2)[label=left:{$Z_1$}, point]; 
% 			\node(Z2) at (2, 2)[label=right:{$Z_2$}, point];
% 			\path (X) edge (Y);
% 			\path (Z1) edge (X);
% 			\path (Z2) edge (Y);
% 			\path[bidirected] (Z1) edge[bend left =10] (Z2);
% 			\draw[gray, fill=gray!30, opacity =.5] (-.1,1.7) rectangle (2.1, 2.3);
% 		\end{tikzpicture} 
% 		\caption*{$(d): Y_x \indep X \mid \*Z$}
% \end{subfigure}
% \end{minipage}
%\vspace{\intextsep}

\begin{minipage}[t]{.32\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering	
		\begin{tikzpicture}[scale = .6]
			\node(X) at (0,0) [label = below:X, point, blue];
			\node(Y) at (2, 0)[label = below:Y, point, red];
			\node[state](Z) at (1, 2) {$\*Z$}; 
			\path (X) edge (Y);
			\path (Z) edge (X);
			\path (Z) edge (Y);
			\path[bidirected] (Z) edge[bend right = 60] (X);
			\path[bidirected] (Z) edge[bend left = 60] (Y);
		\end{tikzpicture} 
		\caption*{$G_{\*C_2}$}
\end{subfigure}
\end{minipage}
\begin{minipage}[t]{.32\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering	
\begin{tikzpicture}[scale = .6]
			\node(X) at (0,0) [label = below:X, point, blue];
			\node(Y) at (2, 0)[label = below:Y, point, red];
			\node(Z1) at (0, 2)[label=left:{$Z_1$}, point]; 
			\node(Z2) at (2, 2)[label=right:{$Z_2$}, point];
			\path (X) edge (Y);
			\path (Z1) edge (X);
			\path (Z1) edge (Y);
			\path (Z2) edge (Y);
			\path (Z2) edge (X);
			\path[bidirected] (Z1) edge[bend right = 60] (X);
			\path[bidirected] (Z2) edge[bend left = 60] (Y);
			\draw[gray, fill=gray!30, opacity =.5] (-.1,1.7) rectangle (2.1, 2.3);
		\end{tikzpicture} 
		\caption*{$(c)$}
\end{subfigure}
\end{minipage}
% \begin{minipage}[t]{.32\linewidth}
% \begin{subfigure}[b]{\linewidth}
% \centering	
% \begin{tikzpicture}[scale = .6]
% 			\node(X) at (0,0) [label = below:X, point, blue];
% 			\node(Y) at (2, 0)[label = below:Y, point, red];
% 			\node(Z1) at (0, 2)[label=left:{$Z_1$}, point]; 
% 			\node(Z2) at (2, 2)[label=right:{$Z_2$}, point];
% 			\path (X) edge (Y);
% 			\path (Z1) edge (X);
% 			\path (Z2) edge (Y);
% 			\path[bidirected] (Z1) edge[bend right = 60] (X);
% 			\path[bidirected] (Z2) edge[bend left = 60] (Y);
% 			\draw[gray, fill=gray!30, opacity =.5] (-.1,1.7) rectangle (2.1, 2.3);
% 		\end{tikzpicture} 
% 		\caption*{$(f): Y_x \indep X \mid \*Z$}
% \end{subfigure}
% \end{minipage}
\begin{minipage}[t]{.32\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering	
\begin{tikzpicture}[scale = .6]
			\node(X) at (0,0) [label = below:X, point, blue];
			\node(Y) at (2, 0)[label = below:Y, point, red];
			\node(Z1) at (0, 2)[label=left:{$Z_1$}, point]; 
			\node(Z2) at (2, 2)[label=right:{$Z_2$}, point];
			\path (X) edge (Y);
			\path (Z1) edge (X);
			\path (Z1) edge (Y);
			\path (Z2) edge (Y);
			\path (Z2) edge (X);
			\path[bidirected] (Z1) edge[bend right = 60] (X);
			\path[bidirected] (Z2) edge[bend left = 60] (Y);
			\path[bidirected] (Z1) edge[bend left =10] (Z2);
			\draw[gray, fill=gray!30, opacity =.5] (-.1,1.7) rectangle (2.1, 2.3);
		\end{tikzpicture} 
		\captionsetup{labelformat=empty}
		\caption*{$(d)$}
\end{subfigure}
\end{minipage}
%\begin{minipage}[t]{.32\linewidth}
% \begin{subfigure}[b]{\linewidth}
% \centering	
% 		\begin{tikzpicture}[scale = .6]
% 			\node(X) at (0,0) [label = below:X, point, blue];
% 			\node(Y) at (2, 0)[label = below:Y, point, red];
% 			\node(Z1) at (0, 2)[label=left:{$Z_1$}, point]; 
% 			\node(Z2) at (2, 2)[label=right:{$Z_2$}, point];
% 			\path (X) edge (Y);
% 			\path (Z1) edge (X);
% % 			\path (Z1) edge (Y);
% 			\path (Z2) edge (Y);
% % 			\path (Z2) edge (X);
% 			\path[bidirected] (Z1) edge[bend right = 60] (X);
% 			\path[bidirected] (Z2) edge[bend left = 60] (Y);
% 			\path[bidirected] (Z1) edge[bend left =10] (Z2);
% 			\draw[gray, fill=gray!30, opacity =.5] (-.1,1.7) rectangle (2.1, 2.3);
% 		\end{tikzpicture} 
% 		\caption*{$(h): Y_x \nindep X \mid \*Z$}
% \end{subfigure}
% \end{minipage}
        \caption{$G_{\*C_1}$ is the C-DAG for diagrams (a) and (b). $G_{\*C_2}$ is the C-DAG for diagrams (c) and (d). $P(y | do(x))$ is identifiable by backdoor adjustment over the cluster $\*Z = \{Z_1, Z_2\}$ in $G_{\*C_1}$ and, therefore, in \emph{all} compatible causal diagrams (e.g., diagrams (a)-(b)).
        However, $P(y | do(x))$ is not identifiable in $G_{\*C_2}$. This means that there is \emph{some} compatible causal diagram for which $P(y | do(x))$ is not identifiable (e.g., diagram (d)).} 
	\label{fig:ignorabilitycluster}
%\vspace{-1.75\intextsep}
\end{figure} 
%\end{wrapfigure} 




==> R-77-CDAGS - AAAI-2023/figs/3_cluster_EC.tex <==
\begin{figure}[t]
%\begin{wrapfigure}{r}{0.35\textwidth}
%\vspace{-2\intextsep}
\begin{minipage}[t]{0.32\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering	
\begin{tikzpicture}[scale = .6]
			\node(X) at (0,0) [label = below:X, point, blue];
			\node(Y) at (2, 0)[label = below:Y, point, red];
			\node[state](Z) at (1, 2) {$\*Z$}; 
			\path (X) edge (Y);
			\path (Z) edge (X);
			\path (Z) edge (Y);
		\end{tikzpicture} 
		\caption*{$G_{\*C_1}$}
\end{subfigure}
\end{minipage}
\begin{minipage}[t]{.32\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering	
\begin{tikzpicture}[scale = .6]
			\node(X) at (0,0) [label = below:$X$, point];
			\node(Y) at (2, 0)[label = below:$Y$, point];
			\node(Z1) at (0, 2)[label=left:{$Z_1$}, point]; 
			\node(Z3) at (2, 2)[label=right:{$Z_3$}, point]; 
			\node(Z2) at (1, 1) {$Z_2$};     %[label=below:{$Z_2$}, point]; 
			\path (X) edge (Y);
			\path (Z1) edge (Z2);
			\path (Z1) edge (X);
			\path (Z3) edge (Z2);
			\path (Z3) edge (Y);
			%\draw[gray, fill=gray!30, opacity =.5] (-.1,1.7) rectangle (2.1, 2.3);
	\end{tikzpicture}
		\caption*{$(a)$}
		%\vspace{0.7em}
\end{subfigure}
\end{minipage}
\begin{minipage}[t]{.32\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering	
\begin{tikzpicture}[scale = .6]
			\node(X) at (0,0) [label = below:$X$, point];
			\node(Y) at (2, 0)[label = below:$Y$, point];
			\node(Z1) at (0, 2)[label=left:{$Z_1$}, point]; 
			\node(Z3) at (2, 2)[label=right:{$Z_3$}, point]; 
			\node(Z2) at (1, 1) {$Z_2$};     %[label=below:{$Z_2$}, point]; 
			\path (X) edge (Y);
			\path (Z1) edge (Z2);
			\path (Z2) edge (Y);
			\path (Z2) edge (X);
			\path (Z1) edge (X);
			\path (Z3) edge (Z2);
			\path (Z3) edge (Y);
			%\draw[gray, fill=gray!30, opacity =.5] (-.1,1.7) rectangle (2.1, 2.3);
	\end{tikzpicture}
		\caption*{$(b)$}
\end{subfigure}
\end{minipage}



\begin{minipage}[t]{.32\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering	
		\begin{tikzpicture}[scale = .6]
			\node(X) at (0,0) [label = below:X, point, blue];
			\node(Y) at (2, 0)[label = below:Y, point, red];
			\node[state](Z) at (1, 2) {$\*Z$}; 
			\path (X) edge (Y);
			%\path (Z) edge (X);
			\path (Z) edge (Y);
			\path[bidirected] (Z) edge[bend right = 60] (X);
			\path[bidirected] (Z) edge[bend left = 60] (Y);
		\end{tikzpicture} 
		\caption*{$G_{\*C_2}$}
\end{subfigure}
\end{minipage}
\begin{minipage}[t]{.32\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering	
\begin{tikzpicture}[scale = .6]
			\node(X) at (0,0) [label = below:$X$, point];
			\node(Y) at (2, 0)[label = below:$Y$, point];
			\node(Z1) at (0, 2)[label=left:{$Z_1$}, point]; 
			\node(Z3) at (2, 2)[label=right:{$Z_3$}, point]; 
			\node(Z2) at (1, 1) {$Z_2$};     %[label=below:{$Z_2$}, point]; 
			\path (X) edge (Y);
			\path (Z1) edge (Z2);
			\path (Z3) edge (Y);
			\path (Z3) edge (Z2);
			%\path (Z3) edge (Y);
			\path[bidirected] (Z1) edge[bend left =20] (Z3);
			\path[bidirected] (Z3) edge[bend left =60] (Y);
			\path[bidirected] (Z1) edge[bend right =60] (X);
			%\draw[gray, fill=gray!30, opacity =.5] (-.1,1.7) rectangle (2.1, 2.3);
	\end{tikzpicture}
		\caption*{$(c)$}
		%\vspace{0.7em}
\end{subfigure}
\end{minipage}	
\begin{minipage}[t]{.32\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering	
\begin{tikzpicture}[scale = .6]
			\node(X) at (0,0) [label = below:$X$, point];
			\node(Y) at (2, 0)[label = below:$Y$, point];
			\node(Z1) at (0, 2)[label=left:{$Z_1$}, point]; 
			\node(Z3) at (2, 2)[label=right:{$Z_3$}, point]; 
			\node(Z2) at (1, 1) {$Z_2$};     %[label=below:{$Z_2$}, point]; 
			\path (X) edge (Y);
			\path (Z1) edge (Z2);
			\path (Z2) edge (Y);
			\path (Z3) edge (Z2);
			%\path (Z3) edge (Y);
			\path[bidirected] (Z1) edge[bend left =20] (Z3);
			\path[bidirected] (Z3) edge[bend left =60] (Y);
			\path[bidirected] (Z1) edge[bend right =60] (X);
			%\draw[gray, fill=gray!30, opacity =.5] (-.1,1.7) rectangle (2.1, 2.3);
	\end{tikzpicture}
		\captionsetup{labelformat=empty}
		\caption*{$(d)$}
\end{subfigure}
\end{minipage}
        \caption{$G_{\*C_1}$ is the C-DAG for diagrams (a) and (b) and $G_{\*C_2}$ is the C-DAG for diagrams (c) and (d), where $\*{Z} = \{Z_1, Z_2, Z_3\}$. $P(y | do(x))$ is identifiable in $G_{\*C_1}$ by backdoor adjustment over $\*Z$ and is not identifiable in $G_{\*C_2}$.} 
	\label{fig:C-EC}
 \vspace{-1\intextsep}	
\end{figure} 
%\vspace{-0.5\intextsep}
%\end{wrapfigure} 




==> R-77-CDAGS - AAAI-2023/figs/3_collapsingGraphs.tex <==
\begin{figure}[t]
%\begin{wrapfigure}{r}{.53\textwidth}
\vspace{-1.5\intextsep}
\begin{minipage}[t]{.32\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering	
\begin{tikzpicture}[scale = .6]
			\node(X) at (0,0) [label = below:$X$, point];
			\node(Y) at (2, 0)[label = below:$Y$, point];
			\node(Z1) at (0, 2)[label=left:{$Z_1$}, point]; 
			\node(Z3) at (2, 2)[label=right:{$Z_3$}, point]; 
			\node(Z2) at (1, 1) {$Z_2$};     %[label=below:{$Z_2$}, point]; 
			\path (X) edge (Y); 
			\path[bend right =30] (Z1) edge (Y);
			\path (Z2) edge (Y);
			\path (Z3) edge (Y);
			\path (Z1) edge (Z2);
			\path (Z2) edge (Z3);
			\path[bidirected] (Z1) edge[bend right =30] (X);
			\path[bidirected] (Z1) edge[bend left =30] (Z2);
			\path[bidirected] (Z2) edge[bend left =30] (Z3);
			\path[bidirected] (Z3) edge[bend left =30] (Y);
	\end{tikzpicture}
		\caption*{$G_1$}
		\vspace{0.0em}
\end{subfigure}
\end{minipage}%	
\begin{minipage}[t]{.32\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering	
\begin{tikzpicture}[scale = .6]
			\node(X) at (0,0) [label = below:$X$, point];
			\node(Y) at (2, 0)[label = below:$Y$, point];
			\node(Z1) at (0, 2)[label=left:{$Z_1$}, point]; 
			\node(Z3) at (2, 2)[label=right:{$Z_3$}, point]; 
			\node(Z2) at (1,1) {$Z_2$};     %[label=below:{$Z_2$}, point]; 
			\path (X) edge (Y);
			\path (Z2) edge (Z1);
			\path (Z2) edge (Z3);
			\path[bidirected] (Z1) edge[bend right =30] (X);
			\path[bidirected] (Z2) edge[bend right =30] (X);
			\path[bidirected] (Z2) edge[bend left =30] (Y);
			\path[bidirected] (Z1) edge[bend left =40] (Z2);
			\path[bidirected] (Z2) edge[bend left =40] (Z3);
			\path[bidirected] (Z3) edge[bend left =30] (Y);
	\end{tikzpicture}
		\caption*{$G_3$}
		\vspace{0.0em}
\end{subfigure}
\end{minipage}%
\begin{minipage}[t]{.32\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering	
\begin{tikzpicture}[scale = .6]
			\node(X) at (0,0) [label = below:$X$, point];
			\node(Y) at (2, 0)[label = below:$Y$, point];
			\node(Z1) at (0, 2)[label=left:{$Z_1$}, point]; 
			\node(Z3) at (2, 2)[label=right:{$Z_3$}, point]; 
			\node(Z2) at (1,1) {$Z_2$};     %[label=below:{$Z_2$}, point]; 
			\path (Y) edge (X);
			\path (Z2) edge (Z1);
			\path (Z2) edge (Z3);
			\path[bend right =30] (Z1) edge (Y); 
			\path (Z2) edge (Y); 
            \path (Z3) edge (Y); 
			\path[bidirected] (Z1) edge[bend right =30] (X);
			\path[bidirected] (Z2) edge[bend right =30] (X);
			\path[bidirected] (Z1) edge[bend left =40] (Z2);
			\path[bidirected] (Z2) edge[bend left =40] (Z3);
	\end{tikzpicture}
		\caption*{$G_5$}
		\vspace{0.0em}
\end{subfigure}
\end{minipage}
% \begin{minipage}[t]{.24\linewidth}
% \begin{subfigure}[b]{\linewidth}
% \centering	
% \begin{tikzpicture}[scale = .6]
% 			\node(X) at (0,0) [label = below:$X$, point];
% 			\node(Y) at (2, 0)[label = below:$Y$, point];
% 			\node(Z1) at (0, 2)[label=left:{$Z_1$}, point]; 
% 			\node(Z3) at (2, 2)[label=right:{$Z_3$}, point]; 
% 			\node(Z2) at (1, 1) {$Z_2$};     
% 			\path[bend right =30] (Z1) edge (Y);
% 			\path (Z2) edge (Y);
% 			\path (Z3) edge (Y);

% 			\path[bidirected] (Z1) edge[bend right =30] (X);
% 			\path[bidirected] (Z1) edge[bend left =30] (Z2);
% 			\path[bidirected] (Z2) edge[bend left =30] (Z3);
% 			\path[bidirected] (Z3) edge[bend left =30] (Y);
% 	\end{tikzpicture}
% 		\caption*{$G_3$}
% 		\vspace{0.0em}
% \end{subfigure}
% \end{minipage}

\begin{minipage}[t]{.32\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering	
\begin{tikzpicture}[scale = .6]
			\node(X) at (0,0) [label = below:$X$, point];
			\node(Y) at (2, 0)[label = below:$Y$, point];
			\node(Z1) at (0, 2)[label=left:{$Z_1$}, point]; 
			\node(Z3) at (2, 2)[label=right:{$Z_3$}, point]; 
			\node(Z2) at (1, 1)   [label=below:{$Z_2$}, point]; % {$Z_2$}; 
			\path (X) edge (Y);
			%\path (Z1) edge (Y);
			\path (Z2) edge (Y);
			\path (Z3) edge (Y);
			\path[bidirected] (Z1) edge[bend right =30] (X);
			\path[bidirected] (Z1) edge[bend left =30] (Z2);
			\path[bidirected] (Z2) edge[bend left =30] (Z3);
			\path[bidirected] (Z3) edge[bend left =30] (Y);
	\end{tikzpicture}
		\caption*{$G_2$}
		\vspace{0.0em}
\end{subfigure}
\end{minipage}	
\begin{minipage}[t]{.32\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering	
\begin{tikzpicture}[scale = .6]
			\node(X) at (0,0) [label = below:$X$, point];
			\node(Y) at (2, 0)[label = below:$Y$, point];
			\node(Z1) at (0, 2)[label=left:{$Z_1$}, point]; 
			\node(Z3) at (2, 2)[label=right:{$Z_3$}, point]; 
			\node(Z2) at (1,1) {$Z_2$};     %[label=below:{$Z_2$}, point]; 
			\path (X) edge (Y);
			\path (Z2) edge (Z1);
			\path (Z2) edge (Z3);
			\path[bidirected] (Z1) edge[bend right =30] (X);
			\path[bidirected] (Z1) edge[bend left =20] (Z3);
			\path[bidirected] (Z3) edge[bend left =30] (Y);
	\end{tikzpicture}
		\caption*{$G_4$}
		\vspace{0.0em}
\end{subfigure}
\end{minipage}
\begin{minipage}[t]{.32\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering	
\begin{tikzpicture}[scale = .6]
			\node(X) at (0,0) [label = below:$X$, point];
			\node(Y) at (2, 0)[label = below:$Y$, point];
			\node(Z1) at (0, 2)[label=left:{$Z_1$}, point]; 
			\node(Z3) at (2, 2)[label=right:{$Z_3$}, point]; 
			\node(Z2) at (1,1) {$Z_2$}; 
			\path (Y) edge (X);
			\path (Z1) edge (Z2);
			\path (Z2) edge (Z3);
			\path (Z3) edge (Y); 
			\path[bidirected] (Z1) edge[bend right =30] (X);
	\end{tikzpicture}
		\caption*{$G_6$}
		\vspace{0.0em}
\end{subfigure}
\end{minipage}

\begin{minipage}[t]{.32\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering	
		\begin{tikzpicture}[scale = .6]
			\node(X) at (0,0) [label = below:X, point, blue];
			\node(Y) at (2, 0)[label = below:Y, point, red];
			\node[state](Z) at (1, 2) {$\*Z$}; 
			\path (X) edge (Y);
			%\path (Z) edge (X);
			\path (Z) edge (Y);
			\path[bidirected] (Z) edge[bend right = 60] (X);
			\path[bidirected] (Z) edge[bend left = 60] (Y);
		\end{tikzpicture} 
		\caption*{$G_{\*C_1}$}
\end{subfigure}
\end{minipage}
% \begin{minipage}[t]{.24\linewidth}
% \begin{subfigure}[b]{\linewidth}
% \centering	
% 		\begin{tikzpicture}[scale = .6]
% 			\node(X) at (0,0) [label = below:X, point, blue];
% 			\node(Y) at (2, 0)[label = below:Y, point, red];
% 			\node[state](Z) at (1, 2) {$\*Z$}; 
% 			\path (Z) edge (Y);
% 			\path[bidirected] (Z) edge[bend right = 60] (X);
% 			\path[bidirected] (Z) edge[bend left = 60] (Y);
% 		\end{tikzpicture} 
% 		\caption*{$G_{\*C_2}$}
% \end{subfigure}
% \end{minipage}
\begin{minipage}[t]{.32\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering	
		\begin{tikzpicture}[scale = .6]
			\node(X) at (0,0) [label = below:X, point, blue];
			\node(Y) at (2, 0)[label = below:Y, point, red];
			\node[state](Z) at (1, 2) {$\*Z$}; 
			\path (X) edge (Y);
			\path[bidirected] (Z) edge[bend right = 60] (X);
			\path[bidirected] (Z) edge[bend left = 60] (Y);
		\end{tikzpicture} 
		\caption*{$G_{\*C_2}$}
\end{subfigure}
\end{minipage}
\begin{minipage}[t]{.32\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering	
		\begin{tikzpicture}[scale = .6]
			\node(X) at (0,0) [label = below:X, point, blue];
			\node(Y) at (2, 0)[label = below:Y, point, red];
			\node[state](Z) at (1, 2) {$\*Z$}; 
			\path (Y) edge (X);
			\path (Z) edge (Y);
			\path[bidirected] (Z) edge[bend right = 60] (X);
		\end{tikzpicture} 
		\caption*{$G_{\*C_3}$}
\end{subfigure}
\end{minipage}

        \caption{With cluster $\*Z = \{Z_1, Z_2, Z_3\}$, $G_{\*C_1}$ is the C-DAG for $G_1$ and $G_2$; $G_{\*C_2}$ is the C-DAG for $G_3$ and $G_4$; and 
        $G_{\*C_3}$ is the C-DAG for $G_5$ and $G_6$. } 
	\label{fig:C-EC2}
\vspace{-1\intextsep}
\end{figure} 
%\end{wrapfigure} 

%
% \begin{minipage}[t]{.24\linewidth}
% \begin{subfigure}[b]{\linewidth}
% \centering	
% \begin{tikzpicture}[scale = .6]
% 			\node(X) at (0,0) [label = below:$X$, point];
% 			\node(Y) at (2, 0)[label = below:$Y$, point];
% 			\node(Z1) at (0, 2)[label=left:{$Z_1$}, point]; 
% 			\node(Z3) at (2, 2)[label=right:{$Z_3$}, point]; 
% 			\node(Z2) at (1, 1) {$Z_2$};     %[label=below:{$Z_2$}, point]; 
% 		%	\path (X) edge (Y);
% 			\path (Z1) edge (Z2);
% 			\path (Z3) edge (Z2);
% 			\path (Z3) edge (Y);

% 			\path[bidirected] (Z1) edge[bend right =30] (X);
% 			\path[bidirected] (Z3) edge[bend left =30] (Y);
% 	\end{tikzpicture}
% 		\caption*{$G_4$}
% 		\vspace{0.0em}
% \end{subfigure}
% \end{minipage}


==> R-77-CDAGS - AAAI-2023/figs/3_med-example.tex <==
\begin{figure}[t]
\begin{subfigure}[b]{0.24\linewidth}
\centering
        \begin{tikzpicture}[scale = .5]
			\node(X) at (0,0) [label = below:$X$, point, blue];
			\node(D) at (0, 2)[label=above:$D$, point]; 
			\node(B) at (.8, 1.1)[label=above:$B$, point]; 
			\node(S) at (1.5, 0)[label=below:$S$, point]; 
			\node(C) at (1.5, 2)[label=above:$C$, point]; 
			\node(A) at (3, 2)[label=above:$A$, point]; 
			\node(Y) at (3, 0)[label = below:$Y$, point, red];
		
			\path (D) edge (X);
			\path (X) edge (S);
			\path (S) edge (Y);
			\path[bidirected] (X) edge[bend right =0] (B); 
		    \path (B) edge (C); 
		    \path (C) edge (Y); 
		    \path[bidirected] (C) edge[bend left = 30] (Y);
		    \path[bidirected] (D) edge[bend left = 30] (C); 
		    \path (A) edge (Y); 
		    \path (A) edge (C); 
        \end{tikzpicture}
        \caption*{$(a)$}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}
\centering
        \begin{tikzpicture}[scale = .5]
            \node(X) at (0,0) [label = below:$X$, point, blue];
% 			\node(D) at (0, 2)[label=left:$D$, point]; 
% 			\node(B) at (.8, .9)[label=below:$B$, point]; 
			\node(S) at (1.5, 0)[label=below:$S$, point]; 
% 			\node[state](SB) at (1.5, 0) {$\{B, S\}$};
% 			\node(C) at (1.5, 2)[label=above left:$C$, point]; 
% 			\node(A) at (3, 2)[label=above:$A$, point]; 
		  %  \node[state](CA) at (1.5, 2) {$\{A, C\}$};
		    \node[state](ABCD) at (1.5, 2) {$\*Z$};
			\node(Y) at (3, 0)[label = below:$Y$, point, red];
		
			\path (ABCD) edge (X);
			\path (X) edge (S);
			\path (S) edge (Y);
			\path[bidirected] (X) edge[bend left =30] (ABCD); 
		  %  \path (S) edge (ABCD); 
		    \path (ABCD) edge (Y); 
		    \path[bidirected] (ABCD) edge[bend left = 30] (Y);
		  %  \path[bidirected] (D) edge[bend left = 30] (CA); 
		  %  \path (ABCD) edge (Y); 
		  %  \path (A) edge (C); 
        \end{tikzpicture}
        \caption*{$(b)$}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}
\centering
        \begin{tikzpicture}[scale = .5]
			\node(X) at (0,0) [label = below:$X$, point, blue];
			\node(D) at (0, 2)[label=above:$D$, point]; 
% 			\node(B) at (.8, .9)[label=below:$B$, point]; 
% 			\node(S) at (1.5, 0)[label=below:$S$, point]; 
			\node[state](SB) at (1.5, 0) {$\*W$};
% 			\node(C) at (1.5, 2)[label=above left:$C$, point]; 
% 			\node(A) at (3, 2)[label=above:$A$, point]; 
		    \node[state](CA) at (1.5, 2) {$\*Z$};
			\node(Y) at (3, 0)[label = below:$Y$, point, red];
		
			\path (D) edge (X);
			\path (X) edge (SB);
			\path (SB) edge (Y);
			\path[bidirected] (X) edge[bend right =30] (SB); 
		    \path (SB) edge (CA); 
		    \path (CA) edge (Y); 
		    \path[bidirected] (CA) edge[bend left = 30] (Y);
		    \path[bidirected] (D) edge[bend left = 30] (CA); 
		    \path (CA) edge (Y); 
		  %  \path (A) edge (C); 
        \end{tikzpicture}
        \caption*{$(c)$}
\end{subfigure}
\begin{subfigure}[b]{0.24\linewidth}
\centering
        \begin{tikzpicture}[scale = .5]
		    \node(X) at (0,0) [label = below:$X$, point, blue];
% 			\node(D) at (0, 2)[label=left:$D$, point]; 
% 			\node(B) at (.8, .9)[label=below:$B$, point]; 
			\node[state](S) at (1.5, 0){$\*W$}; 
% 			\node[state](SB) at (1.5, 0) {$\{B, S\}$};
% 			\node(C) at (1.5, 2)[label=above left:$C$, point]; 
% 			\node(A) at (3, 2)[label=above:$A$, point]; 
		  %  \node[state](CA) at (1.5, 2) {$\{A, C\}$};
		    \node[state](ABCD) at (1.5, 2) {$\*Z$};
			\node(Y) at (3, 0)[label = below:$Y$, point, red];
		
			\path (ABCD) edge (X);
			\path (X) edge (S);
			\path (S) edge (Y);
			\path(S) edge (ABCD);
			\path[bidirected] (X) edge[bend left =30] (ABCD); 
		  %  \path (S) edge (ABCD); 
		    \path (ABCD) edge (Y); 
		    \path[bidirected] (ABCD) edge[bend left = 30] (Y);
		    \path[bidirected] (X) edge[bend right = 30] (S); 
		  %  \path (ABCD) edge (Y); 
		  %  \path (A) edge (C); 
        \end{tikzpicture}
        \caption*{$(d)$}
\end{subfigure}
		\caption{$(a)$: a possible ADMG over %possible causal diagram over
		%of representing the effect of taking lisinopril on having a stroke where 
		lisinopril ($X$), stroke ($Y$), age ($A$), 
		blood pressure ($B$), comorbidities ($C$),  medication history ($D$), and sleep quality ($S$). $(b)$: a C-DAG of $(a)$ with $\*Z=\{A, B, C, D\}$. %where $P(y \mid do(x))$ is identifiable by front-door adjustment. 
		$(c)$: a C-DAG of $(a)$ with $\*W = \{S, B\}$, $\*Z = \{A, C\}$. %where $P(y \mid do(x))$ is not identifiable.
		%(in practice, it would likely not make sense to group the pre-treatment variable of blood pressure with the post-treatment variable of sleep quality).
		% $(d)$: an invalid C-DAG of $(a)$ with $\*W = \{S, B\}, \*Z = \{A, C, D\}$; note %that $\{X, Y, \*W, \*Z\}$ is an inadmissible partition as 
		% a cycle is created among $(X, \*W, \*Z)$.
  $(d)$: an invalid C-DAG of $(a)$, as the partition $\{X, Y, \*W, \*Z\}$, with $\*W = \{S, B\}, \*Z = \{A, C, D\}$ is inadmissible due to the cycle among $(X, \*W, \*Z)$.}
		 \label{fig:med-example}
\vspace{-1\intextsep}		 
\end{figure}












% \begin{figure}[t]
% \begin{center}
% %\begin{multicols}{3}
% \begin{minipage}[t]{.22\columnwidth}
% \centering
% \begin{subfigure}[b]{\linewidth}
% \centering
%         \begin{tikzpicture}[scale = .75]
% 			\node(X) at (0,0) [label = below:$X$, point];
% 			\node(Y) at (3, 0)[label = below:$Y$, point];
% 			\node(C) at (1.7, 2)[label=above left:$C$, point]; 
% 			\node(G) at (1.3, .6)[label=right:$G$, point]; 
% 			\node(D) at (.6, 2)[label=left:$D$, point]; 
% 			\node(A) at (2.5, 2.4)[label=above:$A$, point]; 
% 			\node(B) at (1.5, .2)[label=below:$B$, point]; 
% 			\node(S) at (1.5, -.7)[label=below:$S$, point]; 
% 			\path (X) edge (B);
% 		    \path (X) edge (S);
% 		    \path (B) edge (Y);
% 		    \path (S) edge (Y);
% 			\path (C) edge (X);
% 			\path (C) edge (Y);
% 			\path (G) edge (X);
% 			\path (G) edge (Y);
% 			\path (D) edge (X);
% 			\path (D) edge (Y);
% 			\path (A) edge (C);
% 			\path (A) edge (Y);
% 			\path[bidirected] (C) edge[bend right = 60] (G); 
% 			\path[bidirected] (C) edge[bend left = 60] (A);
% 			\path[bidirected] (C) edge[bend left = 20] (Y);
% 			\path[bidirected] (D) edge[bend right = 30] (X);
%         \end{tikzpicture}
%         \caption*{$(a)$}
% \end{subfigure}
% \end{minipage}
% \begin{minipage}[t]{.22\columnwidth}
% \centering
% \begin{subfigure}[b]{\linewidth}
% \centering
%         \begin{tikzpicture}[scale = .75]
% 			\node(X) at (0,0) [label = below:$X$, point];
% 			\node(Y) at (3, 0)[label = below:$Y$, point];
% % 			\node[state](C) at (.6, 2){$\*C$}; 
% % 			\node(G) at (1.3, .6)[label=right:gender, point]; 
%             \node(W)[state] at (1.7, 0) {$\*W$};
% 			\node(C) at (1.7, 2)[label=above left:$C$, point]; 
% 			\node(D) at (.6, 2)[label=left:$D$, point]; 
% 			\node(A) at (2.5, 2.4)[label=above:$A$, point]; 
% % 			\node(B) at (1.7, .2)[label=below:blood pressure, point]; 
% % 			\node[state](S) at (1.5, -.7){$\*S$}; 
% 			\path (X) edge[bend right = 20] (W);
% 		  %  \path (X) edge (W);
% 		    \path (W) edge (Y);
% 		  %  \path (W) edge (Y);
% 			\path (C) edge (X);
% 			\path (C) edge (Y);
% 			\path (W) edge[bend right = 20]  (X);
% % 			\path (W) edge (Y);
% 			\path (D) edge (X);
% 			\path (D) edge (Y);
% 			\path (A) edge (C);
% 			\path (A) edge (Y);
% 			\path[bidirected] (C) edge[bend right = 20] (W); 
% 			\path[bidirected] (C) edge[bend left = 60] (A);
% 			\path[bidirected] (C) edge[bend left = 20] (Y);
% 			\path[bidirected] (D) edge[bend right = 30] (X);
%         \end{tikzpicture}
%         \caption*{$(b)$}
% \end{subfigure}
% \end{minipage}
% \begin{minipage}[t]{.22\columnwidth}
% \centering
% \begin{subfigure}[b]{\linewidth}
% \centering
%         \begin{tikzpicture}[scale = .75]
% 			\node(X) at (0,0) [label = below:$X$, point];
% 			\node(Y) at (3, 0)[label = below:$Y$, point];
% % 			\node(C) at (2.4, 2)[label=above right:$C$, point]; 
% % 			\node(G) at (1.3, .6)[label=right:$G$, point]; 
% 			\node(D) at (.6, 2)[label=left:$D$, point]; 
% % 			\node(A) at (2.5, 2.4)[label=above:$A$, point]; 
% 			\node[state](W) at (1.5, -.75) {$\*W$};
% 			\node[state](Z) at (2.5, 2) {$\*Z$};
% % 			\node(B) at (1.5, .2)[label=below:$B$, point]; 
% % 			\node(S) at (1.5, -.7)[label=below:$S$, point]; 
% 			\path (X) edge (W);
% 		    \path (X) edge (W);
% 		    \path (W) edge (Y);
% 		    \path (W) edge (Y);
% 			\path (Z) edge (X);
% 			\path (Z) edge (Y);
% 			\path (Z) edge (X);
% 			\path (Z) edge (Y);
% 			\path (D) edge (X);
% 			\path (D) edge (Y);
% % 			\path (Z) edge (C);
% 			\path (Z) edge (Y);
% % 			\path[bidirected] (C) edge[bend right = 60] (Z); 
% % 			\path[bidirected] (C) edge[bend left = 60] (Z);
% 			\path[bidirected] (Z) edge[bend left = 30] (Y);
% 			\path[bidirected] (D) edge[bend right = 30] (X);
%         \end{tikzpicture}
%         \caption*{$(c)$}
% \end{subfigure}
% \end{minipage}
% % \begin{minipage}[t]{.32\columnwidth}
% % \centering
% % \begin{subfigure}[b]{\linewidth}
% % \centering
% %         \begin{tikzpicture}[scale = .8]
% % 			\node(X) at (0,0) [label = left:lisinopril, point];
% % 			\node(Y) at (3, 0)[label = below:stroke, point];
% % 			\node(C) at (.6, 2)[label=left:comorbidities, point]; 
% % 			\node(G) at (1.3, .6)[label=right:gender, point]; 
% % 			\node(D) at (2.5, 2)[label=above:drug history, point]; 
% % 			\node(A) at (1.5, 2.4)[label=above:age, point]; 
% % 			\node(B) at (1.5, .2)[label=below:blood pressure, point]; 
% % 			\node(S) at (1.5, -.7)[label=below:sleep, point]; 
% % 			\path (X) edge (B);
% % 		    \path (X) edge (S);
% % 		    \path (B) edge (Y);
% % 		    \path (S) edge (Y);
% % 			\path (C) edge (X);
% % 			\path (C) edge (Y);
% % 			\path (G) edge (X);
% % 			\path (G) edge (Y);
% % 			\path (D) edge (X);
% % 			\path (D) edge (Y);
% % 			\path (A) edge (C);
% % 			\path (A) edge (Y);
% % 			\path[bidirected] (C) edge[bend right = 20] (G); 
% % 			\path[bidirected] (C) edge[bend left = 30] (A);
% %         \end{tikzpicture}
% %         \caption*{$(a)$}
% % \end{subfigure}
% % \end{minipage}
% \begin{minipage}[t]{.22\columnwidth}
% \centering
% \begin{subfigure}[b]{\linewidth}
% \centering
%         \begin{tikzpicture}[scale = .75]
% 			\node(X) at (0,0) [label = below:$X$, point];
% 			\node(Y) at (3, 0)[label = below:$Y$, point];
% 			\node[state](Z) at (1.5, 2.24) {$\*{Z}$};
% % 			\node[state](Y2) at (3, 0){$\*Y$};
% 			\node[state](W) at (1.5, -.75) {$\*{W}$};
% 			\path (X) edge (W);
% 			\path (W) edge (Y);
% 			\path (Z) edge (Y);
% 			\path (Z) edge (X);
% 			\path[bidirected] (Z) edge[bend right = 30] (X); 
% 			\path[bidirected] (Z) edge[bend left = 30] (Y); 
%         \end{tikzpicture}
%         \caption*{$(d)$}
% \end{subfigure}
% \end{minipage}
%     % \captionsetup{labelformat=empty}
% 		\caption{$(a)$: a causal diagram representing the causal effect of taking lisinopril on having a stroke where $X =$lisinopril, $Y =$ stroke, $A = $age, $B =$ blood pressure, $C$ = comorbidities, $D =$ medication history, $G=$gender, and $S=$sleep quality.$(b)$: an invalid C-DAG of $(a)$ with $\*W = \{S, B, G\}$. $(c)$: a valid C-DAG of $(a)$ where $\*W = \{S, B\}, \*Z=\{A, C, G\}$ that is identifiable by both the back-door and front-door. $(d)$: a valid C-DAG of $(a)$ where $\*W = \{S, B\}, \*Z = \{A, C, D, G\}$, that is not identifiable by the backdoor. \xcomment{we could have (b) as the last one.}}
% 		 \label{fig:med-example}
% \end{center}
% \end{figure}


==> R-77-CDAGS - AAAI-2023/figs/a1_multipleXY.tex <==
\begin{figure}[h!]
\begin{minipage}[t]{.24\columnwidth}
\centering
\begin{subfigure}[b]{\linewidth}
\centering
        \begin{tikzpicture}[scale = 0.5]
			\node(X1) at (0,0) [label = below:$X_1$, point, blue];
			\node(X2) at (1.5, 0)[label=above:$X_2$, point, blue]; 
			\node(Y2) at (3, 0)[label = below:$Y_2$, point, red];
		    \node(Y1) at (1.5, -1)[label=below:$Y_1$, point, red]; 
			\path (X1) edge (X2);
			\path (X2) edge (Y1);
			\path (X2) edge (Y2);
			\path (X1) edge (Y1);
			\path (Y1) edge (Y2);
			\path[bidirected] (X1) edge[bend left =70] (Y2); 
        \end{tikzpicture}
        \caption*{$(a)$ $G_1$}
\end{subfigure}
\end{minipage}
\begin{minipage}[t]{.24\columnwidth}
\centering
\begin{subfigure}[b]{\linewidth}
\centering
        \begin{tikzpicture}[scale = 0.5]
			\node(X1) at (0,0) [label = below:$X_1$, point, blue];
			\node(X2) at (1.5, 0)[label=above:$X_2$, point, blue]; 
			\node(Y2) at (3, 0)[label = below:$Y_2$, point, red];
		    \node(Y1) at (1.5, -1)[label=below:$Y_1$, point, red]; 
			\path (X1) edge (X2);
			\path (X2) edge (Y1);
			\path (X2) edge (Y2);
			\path (X1) edge (Y1);
			\path (Y1) edge (Y2);
			\path[bidirected] (X1) edge[bend left =30] (X2); 
			\path[bidirected] (X1) edge[bend left =70] (Y2); 
        \end{tikzpicture}
        \caption*{$(b)$ $G_2$}
\end{subfigure}
\end{minipage}
\begin{minipage}[t]{.24\columnwidth}
\centering
\begin{subfigure}[b]{\linewidth}
\centering
        \begin{tikzpicture}[scale = 0.5]
			\node(X1) at (0,0) [label = below:$X_1$, point, blue];
			\node(X2) at (1.5, 0)[label=above:$X_2$, point, blue]; 
			\node(Y2) at (3, 0)[label = below:$Y_2$, point, red];
		    \node(Y1) at (1.5, -1)[label=below:$Y_1$, point, red]; 
			\path (X1) edge (X2);
			\path (X2) edge (Y1);
			\path (X2) edge (Y2);
			\path (X1) edge (Y1);
			%\path (Y1) edge (Y2);
			\path[bidirected] (X1) edge[bend left =70] (Y2); 
			\path[bidirected] (Y1) edge[bend right =0] (Y2); 
        \end{tikzpicture}
        \caption*{$(c)$ $G_3$}
\end{subfigure}
\end{minipage}
\begin{minipage}[t]{.24\columnwidth}
\centering
\begin{subfigure}[b]{\linewidth}
    \begin{minipage}[b][1.5cm][t]{\columnwidth}
    \centering
    \begin{tikzpicture}[scale = 0.5]
        \node[state, blue](X) at (0, 2){$\*X$}; 
 		\node[state, red](Y) at (2, 2) {$\*Y$};
		\path (X) edge (Y);
		\path[bidirected] (X) edge[bend left =60] (Y); 
    \end{tikzpicture}
    \end{minipage}
    \caption*{$(d)$ $G_{\*C}$}
\end{subfigure}
\end{minipage}
    % \captionsetup{labelformat=empty}
		\caption{$(a), (b),$ and $(c)$ are causal diagrams compatible with the C-DAG $G_\*C$ in $(d)$ where $\*X = \{X_1, X_2\}$ and $\*Y = \{Y_1, Y_2\}$. The causal effect $P(y_1, y_2 | do(x_1, x_2))$ is identifiable in $(a)$ but not in $(b)$ or $(c)$. Consequently, the effect $P(\*y | do(\*x))$ is not identifiable from the C-DAG $G_\*C$.}
		 \label{fig:a1_multipleXY}
\end{figure}







==> R-77-CDAGS - AAAI-2023/figs/a2_multipleXY.tex <==
\begin{figure}[h!]
\begin{center}
\begin{minipage}[t]{.28\columnwidth}
\begin{subfigure}[b]{\linewidth}
\centering
        \begin{tikzpicture}[scale = .5]
			\node(X1) at (0,0) [label = below:$X_1$, point, blue];
			\node(X2) at (1.25,0)[label=below:$X_2$, point, blue];
		    \node(Y1) at (2.5, 0)[label=below:$Y_1$, point, red];
			\node(Y2) at (3.75, 0)[label = below:$Y_2$, point, red];
		    \node(Z1) at (1.25, 1.5)[label=above:$Z_1$, point];
			\node(Z2) at (2.5, 1.5)[label = above:$Z_2$, point];
			\path (X1) edge (X2);
			\path (X2) edge (Y1);
			\path (Y1) edge (Y2);
			\path (Z1) edge (Y1);
			\path (Z2) edge (X2);
			\path[bidirected] (Y1) edge[bend left =30] (Y2); 
			\path[bidirected] (Z1) edge[bend left =0] (X1); 
			\path[bidirected] (Z2) edge[bend left =0] (Y2); 
        \end{tikzpicture}
        \caption*{$(a)$ $G$}
\end{subfigure}
\end{minipage}
\begin{minipage}[t]{.22\columnwidth}
\begin{subfigure}[b]{\linewidth}
    \begin{minipage}[b][1.8cm][t]{\columnwidth}
    \centering
    \begin{tikzpicture}[scale = .5]
        \node[state, blue](X) at (0, 0){$\*X$}; 
 		\node[state, red](Y) at (1.8, 0) {$\*Y$};
		\node[state](Z) at (0.9, 2.2) {$\*Z$};
		\path (X) edge (Y);
		\path (Z) edge (X);
		\path (Z) edge (Y);
		\path[bidirected] (Z) edge[bend left =30] (Y); 
		\path[bidirected] (Z) edge[bend right =30] (X); 
    \end{tikzpicture}
    \end{minipage}
    \caption*{$(b)$ $G_{\*C_1}$}
\end{subfigure}
\end{minipage}
\begin{minipage}[t]{.22\columnwidth}
\begin{subfigure}[b]{\linewidth}
    \begin{minipage}[b][1.8cm][t]{\columnwidth}
    \centering
    \begin{tikzpicture}[scale = .5]
        \node[state, blue](X) at (0, 0){$\*X$}; 
 		\node[state, red](Y) at (2.5, 0) {$\*Y$};
	    \node(Z1) at (0.625, 1.5)[label=above:$Z_1$, point];
		\node(Z2) at (1.775, 1.5)[label = above:$Z_2$, point];
		\path (X) edge (Y);
		\path (Z1) edge (Y);
		\path (Z2) edge (X);
		\path[bidirected] (Z2) edge[bend left =0] (Y); 
		\path[bidirected] (Z1) edge[bend right =0] (X); 
    \end{tikzpicture}
    \end{minipage}
    \caption*{$(c)$ $G_{\*C_2}$}
\end{subfigure}
\end{minipage}
\begin{minipage}[t]{.22\columnwidth}
\centering
\begin{subfigure}[b]{\linewidth}
    \begin{minipage}[b][1.8cm][t]{\columnwidth}
    \centering
    \begin{tikzpicture}[scale = .5]
		\node(X1) at (0,0) [label = below:$X_1$, point, blue];
		\node(X2) at (1.25,0)[label=below:$X_2$, point, blue];
 		\node[state, red](Y) at (2.5, 0) {$\*Y$};
		\node[state](Z) at (1.25, 2.2) {$\*Z$};
		\path (X1) edge (X2);
		\path (X2) edge (Y);
		\path (Z) edge (X2);
		\path (Z) edge (Y);
		\path[bidirected] (Z) edge[bend left =30] (Y); 
		\path[bidirected] (Z) edge[bend right =30] (X1); 
    \end{tikzpicture}
    \end{minipage}
    \caption*{$(d)$ $G_{\*C_3}$}
\end{subfigure}
\end{minipage} 
		\caption{$(a)$: causal diagram $G$ where the effect $P(y_1, y_2 | do(x_1, x_2))$ is identifiable. $(b)$: C-DAG $G_{\*C_1}$ 
% 		resulting from 
		with clustering $\*X = \{X_1, X_2\}$, $\*Y = \{Y_1, Y_2\}$, and $\*Z = \{Z_1, Z_2\}$. $(c)$: C-DAG $G_{\*C_2}$ 
% 		resulting from 
		with clustering $\*X = \{X_1, X_2\}$ and $\*Y = \{Y_1, Y_2\}$. $(d)$: C-DAG $G_{\*C_3}$ 
% 		resulting from 
		with clustering $\*Y = \{Y_1, Y_2\}$ and $\*Z = \{Z_1, Z_2\}$. The effect $P(\*y | do(\*x))$ is not identifiable in $G_{\*C_1}$, but 
% 		$P(\*y | do(\*x))$ 
		is identifiable in $G_{\*C_2}$ and $P(\*y | do(x_1, x_2))$ is identifiable in $G_{\*C_3}$.}
		 \label{fig:a2_multipleXY}
\end{center}
\vspace{-0.5\intextsep}
\end{figure}







==> R-77-CDAGS - AAAI-2023/figs/clusters_path_analysis.tex <==
%\begingroup
%\begin{wrapfigure}{r}{0.35\textwidth}
%\vspace{-2\intextsep}
\begin{figure*}[t]
\begin{minipage}[t]{.24\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering	
\begin{tikzpicture}[scale = 0.85]
			\node[state](Z) at (0,0) {$\*{Z}$};
			\node[state](X) at (-1.1, 0){$\*{X}$};%[label = left:X, point];
			\node[state](Y) at (1.1, 0){$\*{Y}$};%[label=right:Y, point]; 
			\path[{Rays[n=6]}-Latex] (X) edge (Z);
            % \path(X) edge (Z);
			\path (Z) edge (Y);
		\end{tikzpicture}
		\vspace{+0.15in}
		\caption*{$(a)$}
        \vspace{+0.1in}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
		\begin{tikzpicture}[scale = 0.85]
			\node(X) at (-1.7, 0)[label = below:X, point];
			\node(Y) at (1.7, 0)[label=below:Y, point]; 
			\node(Z2) at (0,0) {$Z_2$};
			\node(Z1) at (-.9,0) {$Z_1$};
			\node(Z3) at (.9,0) {$Z_3$};
			\path (X) edge (Z1);
			\path (Z3) edge (Y);
			\path (Z1) edge (Z2);
			\path (Z2) edge (Z3);
		\end{tikzpicture}
		\vspace{+0.01in}
		\caption*{$(b)$}
		\vspace{+0.05in}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
\centering		
		\begin{tikzpicture}[scale = 0.85]
			\node(X) at (-1.7, 0)[label = below:X, point];
			\node(Y) at (1.7, 0)[label=below:Y, point]; 
			\node(Z2) at (0,0) {$Z_2$};
			\node(Z1) at (-.9,0) {$Z_1$};
			\node(Z3) at (.9,0) {$Z_3$};
			\path (X) edge (Z1);
			\path (Z3) edge (Y);
			\path (Z1) edge (Z2);
			\path (Z3) edge (Z2);
		\end{tikzpicture}
		\vspace{+0.01in}
		\caption*{$(c)$}
\end{subfigure}
\end{minipage}
\hfill\vline\hfill
\begin{minipage}[t]{.24\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering
\begin{tikzpicture}[scale = 0.85]
			\node[state](Z) at (0,0) {$\*{Z}$};
			\node[state](X) at (-1.1, 0){$\*{X}$};%[label = left:X, point];
			\node[state](Y) at (1.1, 0){$\*{Y}$};%[label=right:Y, point]; 
			\path (Z) edge (X);
			\path (Z) edge (Y);
		\end{tikzpicture}
		\vspace{+0.15in}
        \caption*{$(d)$}
        \vspace{+0.1in}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
\centering
		\begin{tikzpicture}[scale = 0.85]
			\node(X) at (-1.7, 0)[label = below:X, point];
			\node(Y) at (1.7, 0)[label=below:Y, point]; 
			\node(Z2) at (0,0) {$Z_2$};
			\node(Z1) at (-.9,0) {$Z_1$};
			\node(Z3) at (.9,0) {$Z_3$};
			\path (Z1) edge (X);
			\path (Z3) edge (Y);
			\path (Z1) edge (Z2);
			\path (Z2) edge (Z3);
		\end{tikzpicture}
			\vspace{+0.01in}
	        \caption*{$(e)$}
	        \vspace{+0.05in}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
\centering
		\begin{tikzpicture}[scale = 0.85]
			\node(X) at (-1.7, 0)[label = below:X, point];
			\node(Y) at (1.7, 0)[label=below:Y, point]; 
			\node(Z2) at (0,0) {$Z_2$};
			\node(Z1) at (-.9,0) {$Z_1$};
			\node(Z3) at (.9,0) {$Z_3$};
			\path (Z1) edge (X);
			\path (Z3) edge (Y);
			\path (Z1) edge (Z2);
			\path (Z3) edge (Z2);
		\end{tikzpicture}
		\vspace{+0.01in}
	 \caption*{$(f)$}
\end{subfigure}
\end{minipage}
\hfill\vline\hfill
\begin{minipage}[t]{.24\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering
\begin{tikzpicture}[scale = 0.85]
			\node[state](Z) at (0,0) {$\*{Z}$};
			\node[state](X) at (-1.1, 0){$\*{X}$};%[label = below:X, point];
			\node[state](Y) at (1.1, 0){$\*{Y}$};%[label=below:Y, point]; 
			\path[{Rays[n=6]}-Latex] (X) edge (Z);
			\path[{Rays[n=6]}-Latex] (Y) edge (Z);
		\end{tikzpicture}
\vspace{+0.15in}
\caption*{$(g)$}
\vspace{+0.1in}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
\centering
		\begin{tikzpicture}[scale = 0.85]
			\node(X) at (-1.5, 0)[label = below:X, point];
			\node(Y) at (1.5, 0)[label=below:Y, point]; 
			\node(Z1) at (0,0) {$Z_1$};
			\node(Z2) at (0,-.9) {$Z_2$};
			\node(Z3) at (.9,-.9) {$Z_3$};
			\path (X) edge (Z1);
			\path (Y) edge (Z1);
			\path (Z1) edge (Z2);
			\path (Z3) edge (Z2);
		\end{tikzpicture}
\caption*{$(h)$}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
%\vspace{+0.1in}
\centering
		\begin{tikzpicture}[scale = 0.85]
			\node(X) at (-1.7, 0)[label = below:X, point];
			\node(Y) at (1.7, 0)[label=below:Y, point]; 
			\node(Z2) at (0,0) {$Z_2$};
			\node(Z1) at (-.9,0) {$Z_1$};
			\node(Z3) at (.9,0) {$Z_3$};
			\path (X) edge (Z1);
			\path (Y) edge (Z3);
			\path (Z1) edge (Z2);
			\path (Z2) edge (Z3);
		\end{tikzpicture}
		\vspace{+0.01in}
	\caption*{$(i)$}
\end{subfigure}
\end{minipage}
\hfill\vline\hfill
\begin{minipage}[t]{.24\linewidth}
\begin{subfigure}[b]{\linewidth}
\centering
 \begin{tikzpicture}[scale = 0.85]
			\node[state](Z) at (0,-1) {$\*{Z}$};
			\node[state](X) at (-1.2, 0){$\*{X}$};%[label = below:X, point];
			\node[state](Y) at (1.2, 0){$\*{Y}$};%[label=below:Y,
			\node(W)[state] at (0, 0) {$\*{W}$}; %[label=above:W, point]; 
			\path (X)[{Rays[n=6]}-Latex] edge (W);
			\path (Y)[{Rays[n=6]}-Latex] edge (W);
			\path (W) edge(Z);
		\end{tikzpicture} 
\caption*{$(j)$}
%\vspace{+0.1in}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
\centering
		\begin{tikzpicture}[scale = 0.85]
			\node(X) at (-1, 0)[label = below:$X$, point];
			\node(W1) at (0, 0) {$W_1$}; 
			\node(W2) at (1, 0) {$W_2$}; 
			\node(Y) at (2, 0)[label=below:$Y$, point]; 
			\node(Z1) at (0,-.9) {$Z1$};
			\node(Z2) at (1,-.9) {$Z2$};
			\path (X) edge (W1);
			\path (Y) edge (W2);
			\path (W2) edge (W1); 
			\path (W1) edge (Z1);
			\path (Z2) edge (Z1);
		\end{tikzpicture}
\caption*{$(k)$}
%\vspace{+0.1in}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
\centering
		\begin{tikzpicture}[scale = 0.85]
			\node(X) at (-1, 0)[label = below:$X$, point];
			\node(W1) at (0, 0) {$W_1$}; 
			\node(W2) at (1, 0) {$W_2$}; 
			\node(Y) at (2, 0)[label=below:$Y$, point]; 
			\node(Z1) at (0,-.9) {$Z1$};
			\node(Z2) at (1,-.9) {$Z2$};
			\path (X) edge (W1);
			\path (Y) edge (W2);
			\path (W1) edge (W2); 
			\path (W1) edge (Z1);
			\path (Z2) edge (Z1);
		\end{tikzpicture}
\caption*{$(l)$}
\end{subfigure}
\end{minipage}
		\caption{Causal diagrams $(b), (c)$ are compatible with the C-DAG $(a)$. Causal diagrams $(e), (f)$ are compatible with the C-DAG $(d)$. In C-DAGs $(a), (d)$, $\*{Z}$ is a non-collider between $\*{X}$ and $\*{Y}$. 
		The path is active in $(b), (e)$, but inactive in $(c)$ and $(f)$.
		Causal diagrams $(h),(i)$ are compatible with the C-DAG $(g)$, where $\*{Z}$ is a collider between $\*{X}$ and $\*{Y}$. Causal diagrams $(k),(l)$ are compatible with the C-DAG $(j)$, where $\*{W}$ is a collider between $\*{X}$ and $\*{Y}$, and $\*{Z}$ is a descendant of $\*{W}$. When $\*{Z}$ is conditioned on, the path is active in $(h), (k)$, but inactive in $(i), (l)$.}
	\label{fig:clusterPathAnalysis}
%\vspace{-1\intextsep}
\end{figure*}
%\endgroup

==> R-77-CDAGS - AAAI-2023/sections/01_introduction.tex <==
\section{Introduction}

% 1. usefulness of causality 
% 2. id problem and ample literature , do-calc and id algorithms 
% 3. challenging for its applicability 
% 4. 

One of the central tasks found in data-driven disciplines is to infer the effect of a treatment $X$ on an outcome $Y$, which is formally written as the interventional distribution $P(Y | do(X=x))$, from observational (non-experimental) data collected from the phenomenon under investigation. These relations are considered essential in the construction of explanations and for making decisions about interventions that have never been implemented before  \citep{pearl:2k,spirtes:etal00,bareinboim:pea16,PetersJanzingSchoelkopf17}.%,pearl:mackenzie2018}.  

Standard tools necessary for identifying the aforementioned  do-distribution, such as d-separation, do-calculus \cite{pearl:95a}, and the ID-algorithm \cite{tian:pea02-general-id,shpitser:pea06a,huang:val06-complete, lee:etal19} take as input a combination of an observational distribution and a qualitative description of the underlying causal system, often articulated in the form of a causal diagram \citep{pearl:2k}. However,  specifying a causal diagram requires knowledge about the causal relationships among all pairs of observed variables, which is not always available in many real-world applications. This is especially  true and acute in complex, high-dimensional settings, which curtails the applicability of causal inference theory and tools.
%galles:pea95,
%Intuitively, a causal diagram $G$ has a directed edge from $X$ to $Y$ %(e.g., see Fig.\ref{fig:ignorabilitycluster}(a)) 
%if $Y$ ``listens'' to the value of $X$; in terms of the underlying causal system, $X$ appears as an argument of the mechanism of $Y$.  The importance of this notion has been emphasized in the literature by Pearl: ``This listening metaphor encapsulates the entire knowledge that a causal network conveys; the rest can be derived, sometimes by leveraging data''  \citep[p.~129]{pearl:mackenzie2018}.
% %This construction produces a coarsening of the underlying mechanisms such that the arguments of the functions are preserved while their particular forms are discarded, which is sometimes known as non-parametric. 

%Once the causal diagram is fully articulated based on domain knowledge, the empirical researcher can use standard causal inference tools to infer the effect of a treatment $X$ on an outcome $Y$, which is formally written as the interventional distribution $P(Y | do(X=x))$. Determining whether the do-distribution is inferable from the combination of the causal diagram $G$  and the observational distribution $P(\*V)$, where $\*V$ represents the set of observed variables, is known as the \textit{identification problem}. This problem has been extensively studied, with proposed approaches including  
%and a number of conditions have been proposed. These include 
%symbolic methods such as Pearl's celebrated do-calculus \cite{pearl:95a} as well as algorithmic strategies \cite{galles:pea95,tian:pea02-general-id,shpitser:pea06a,huang:val06-complete, lee:etal19}. %, to cite a few. 
%Despite the power of such approaches, limited scientific knowledge may hinder the full specification of causal diagrams, 
 %In fields like medicine, for example, there may be significant observational data available, and comparatively limited domain knowledge contextualizing how each of the variables in the dataset causally relate to each other. 
 In the context of medicine, for example, electronic health records include data on lab tests, %conditions observed, 
drugs, demographic information, and other clinical attributes, but medical knowledge is not yet advanced enough to lead to the construction of causal diagrams over all of these variables, limiting the use of the graphical approach to inferring causality \cite{kleinberg_review_2011}. In many cases, however, contextual or temporal information about variables is available, which may partially inform how these variables are situated in a causal diagram relative to other key variables. For instance, a data scientist may know that covariates
%variables like age ($A$), blood pressure ($B$), comorbidities ($C$), and medication history ($D$) 
occur temporally before a drug is prescribed or an outcome occurs. They may even suspect that some pre-treatment variables are causes of the treatment and the outcome variables. However, they may be uncertain about the relationships among each pair of covariates, or it may be burdensome to explicitly define them. Given that a misspecified causal diagram may lead to wrong causal conclusions, this issue raises the question of whether a coarser representation of the causal diagram, where no commitment is made to the relationship between certain variables, would still be sufficient to determine the causal effect of interest. 

% which we will defined as a cluster. %, by what we will define as a cluster. 


In this paper, our goal is to develop a framework for %identification of causal effects 
causal inferences
in partially understood domains such as the medical domain discussed above. 
% First, we introduce a novel graphical model that allows the specification of the causal relationships over clusters of variables, while the relationships among the variables within the clusters are left unspecified. 
%\hl{Change next discussion}
We will focus on formalizing the problem of causal effect identification considering that the data scientist does not have prior knowledge to fully specify a causal diagram %or causal relationships 
over all pairs of variables.
%, but does have prior knowledge to % specify the causal relationships over clusters or groupings of variables. partially specify causal relationships between variables in different clusters or groups. 
First, we formally define and characterize %a novel causal graphical model 
a novel class of graphs
called \textit{cluster DAGs} (or C-DAG, for short), which will allow for encoding of partially understood causal relationships between variables in different abstracted clusters, representing a group of variables among which causal relationships are not %fully 
understood or specified. 
%Within a cluster, any relationships between variables are possible, so a C-DAG represents an equivalence class of causal diagrams compatible with the knowledge available.
%Such a model can be considered an equivalence class of graphical models, allowing for ambiguity in the specification of the relationships within clusters. 
Then, we develop the foundations and machinery for valid probabilistic and causal inferences, akin to Pearl’s d-separation and do-calculus for when such a coarser graphical representation of the system is provided based on the limited prior knowledge available. 
In particular, we follow Pearl's Causal Hierarchy \citep{pearl:mackenzie2018, bar:etal2020} and develop the machinery for inferences in C-DAGS at all three inferential layers -- $\mathcal{L}_1$ (associational), $\mathcal{L}_2$ (interventional), and $\mathcal{L}_3$ (counterfactual).
%\xadd{Then, following Pearl's causal hierarchy, we show that a C-DAG is optimal for inferences over clusters (macro-variables) at all three inferential layers -- $\mathcal{L}_1$ (associational), $\mathcal{L}_2$ (interventional), and $\mathcal{L}_3$ (counterfactual). Specifically, we show that a C-DAG is a (probabilistic) Bayesian Network (BN) over macro-variables and d-separation is sound and complete for extracting conditional independence relations over such macro-variables. Moreover, we show that a C-DAG is a Causal Bayesian Network (CBN) over macro-variables and causal tools such as do-calculus and ID algorithm are sound and complete for causal reasoning over such macro-variables. Finally, we show that a C-DAG is induced by a Structural Causal Model (SCM) over macro-variables which is equivalent to the underlying SCM over the original variables on statements about the macro-variables. Therefore, tools for counterfactual reasoning are also sound and complete in C-DAGs (?)} 
%, akin to Pearl’s d-separation and do-calculus for when such a coarser graphical representation of the system is provided based on the limited prior knowledge available.
%\footnote{Investigating different structure learning approaches for the full DAG is not part of the scope of this paper.}
The results  are fundamental first steps in terms of semantics and graphical conditions to perform probabilistic, interventional, and counterfactual inferences over clusters of variables. %The new proposed semantics provide the basis for the development of more practical and relaxed causal inferences and learning tools.
%@Adele-write future research direction in the end
%\footnote{A future research direction is to develop learning algorithms to assist the construction of cluster causal diagrams from data, but is out of scope for this work.}

%\xst{In particular, to allow for more refined groupings of variables, we introduce a new class of graphical models over a set of clusters of variables, where the relationships amongst variables within a cluster are left unspecified. Further, we develop machinery for valid causal inference in such models.}  
%The proposed method enables valid causal inference with a partial understanding of the relationships among variables. 
%In this paper, we bridge the gap between requiring a full specification of the system and clustering all covariates together while ignoring what is within the cluster. In particular, to allow for  more refined grouping of variables, we introduce a new class of graphical models over a set of clusters of variables  where the relationships amongst variables within the cluster are left unspecified. We develop machinery for valid causal inference in such models.  The proposed method enables valid causal inference with a partial understanding of the relationships among variables. 
%In this paper, our goal is to strike a balance between these approaches and allow for a coarser way of specifying assumptions while \xst{developing} \xadd{leveraging} machinery that preserves the validity of the inferences.  For concreteness, consider the graphs in Figs.~\ref{fig:ignorabilitycluster}(c) and (f). We note that $P(Y | do(X))$ is identifiable in both cases, \textit{regardless} of the relationship among the $\*Z$ nodes. We would like to identify such cases in which the full specification of the system is not needed, while being cognizant of the  implications of leaving the relationships within a cluster unspecified.  
%We will introduce a new class of graphical models, coarser than causal diagrams, and develop machinery that allows us to evaluate the validity of the inferences within this class.  
Specifically, we outline our technical contributions below. %in the following.
%\xcomment{Write the contributions emphasizing better what is done, maybe adding references to the Theorem.}
%\input{figs/1_fig1_compact}
%\vspace{-0.5em}
%\hl{change the list of contributions}
\begin{enumerate}
\setlength\itemsep{0em}
    \item We introduce a new graphical modelling tool called \emph{cluster DAGs} (or C-DAGs) over %a set of
    macro-variables representing clusters of variables where the relationships among the variables inside the clusters are left unspecified \textit{(Definition \ref{def:cdag})}. %We show that interventional distributions admit a convenient factorization following the coarser structure of C-DAGs. This gives a C-DAG the semantics of an equivalence class of all compatible underlying causal diagrams \textit{(Theorem \ref{thm:markovrelative})}.
    Semantically, a C-DAG represents an equivalence class of all %compatible
    underlying graphs over the original variables that share the relationships among the clusters.
   % \item We show that 
  
  \item We show that a C-DAG is a (probabilistic) Bayesian Network (BN) over macro-variables and Pearl's d-separation is sound and complete for extracting conditional independencies over macro-variables if the underlying graph over the original variables is a BN (\textit{Theorems \ref{thm:dsep_cdag_dag} and  \ref{thm:cdag_bn}}).
    
%    \item We prove the soundness and completeness of Pearl's d-separation and do-calculus rules extended to the coarse graphical representation of  C-DAGs \textit{(Theorems \ref{thm:dsep_cdag_dag}, \ref{thm:docalc-cdags} and \ref{thm:do-calc_completenes})}, despite C-DAGs’ abstracted representation of possibly numerous underlying causal diagrams.
    
  \item We show that a C-DAG is a Causal Bayesian Network (CBN) over macro-variables and Pearl's do-calculus is sound and complete for causal inferences about macro-variables in C-DAGs if the underlying graph over the original variables is a CBN (\textit{Theorems \ref{thm:docalc-cdags}, \ref{thm:do-calc_completenes}, and \ref{thm:markovrelative}}).  The results can be used to show that the ID-algorithm is sound and complete to systematically infer causal effects from the  observational distribution and partial domain knowledge encoded as a C-DAG (\textit{Theorem \ref{thm:ids}}). 
%    \item %Given the developed language and foundations of C-DAGs, we prove that the ID-algorithm is sound and complete to systematically infer causal effects from the %combination of an 
    %observational distribution and partial domain knowledge encoded as a C-DAG \textit{(Theorem \ref{thm:ids})}. 
% \item    We prove that interventional distributions admit a convenient factorization following the C-DAG's structure \textit{(Theorem \ref{thm:markovrelative})}. This factorization can be used to show that the ID-algorithm is sound and complete to systematically infer causal effects from the  observational distribution and partial domain knowledge encoded as a C-DAG \textit{(Theorem \ref{thm:ids})}.
\item We show that, assuming the underlying graph $G$ is induced by an SCM $\mathcal{M}$, then 
there exists an SCM $\mathcal{M}_{\*C}$ over macro-variables $\*C$ such that its induced causal diagram is $G_{\*C}$ and it is equivalent to $\mathcal{M}$ on statements about the macro-variables (\textit{Theorem~\ref{thm:ctf_cdags}}). Therefore, the CTFID algorithm \citep{correa21nestedctf} for the identification of nested counterfactuals from an arbitrary combination of observational and experimental distributions can be extended to the C-DAGs.

%and,a C-DAG is induced by a Structural Causal Model (SCM) over macro-variables which is equivalent to the underlying SCM over the original variables on statements about the macro-variables. Therefore, tools for counterfactual reasoning are also sound and complete in C-DAGs
    \end{enumerate}

%\input{figs/3_med-example}

%     \item We introduce a new class of graphs called cluster DAGs (or C-DAGs) over a set of clusters of variables where the relationships amongst the variables inside the clusters are left unspecified \textit{(Definition \ref{def:cdag})}.
%     \item We show that despite C-DAGs' abstracted representation of %numerous possible 
%     possibly numerous 
%     underlying paths, separation rules can be developed to account for the clusters. We prove the soundness and completeness of the d-separation rules extended to C-DAGs \textit{(Theorem \ref{thm:dsep_cdag_dag})}. 
%     \item We prove that the inference rules known as Pearl's do-calculus are sound and complete for the coarse representation of C-DAGs \textit{(Theorems \ref{thm:docalc-cdags} and \ref{thm:do-calc_completenes})}.
%     \item  We prove that interventional distributions admit a convenient factorization following the C-DAG's structure \textit{(Theorem \ref{thm:markovrelative})}. This factorization can be used to show that the ID-algorithm is sound and complete to systematically infer causal effects from the combination of an observational distribution and partial domain knowledge encoded as a C-DAG \textit{(Theorem \ref{thm:ids})}. 

%\vspace{-0.2in}
\subsection{Related work}

%\xadd{There are other attempts in the literature to address the difficulty of specifying a full causal diagram.  the work by Beckers and Halpern (AAAI 19) and other recent work on causal abstraction. }
Since a group of variables may constitute a semantically meaningful entity, causal models over abstracted clusters of variables have attracted increasing attention for the development of more interpretable tools \cite{scholkopf2021toward,Shen2018psdd}.
\cite{parviainen16groupbn} studied the problem of, given a DAG, under what assumptions a DAG over macro-variables can represent
the same conditional independence relations between the macro-variables. 
%\cite{Shen2018psdd} mentioned the use of Bayesian network (BN) over clusters of variables.
Recent developments on causal abstraction  %, however, 
have focused on the distinct problem of investigating %functions that map 
mappings of a cluster of (micro-)variables to a single (macro-)variable, while preserving some causal properties \citep{chalupka15visual, chalupka16multi, rubensteinWBMJG17, halpern19abstraction}. %and, importantly, assuming a structural causal model defined on the level on which the variables were measured, is given. 
The result is a new structural causal model defined on a higher level of abstraction, but with causal properties similar to those in the low-level model.\footnote{In \cite{halpern19abstraction}'s notation, we investigate the case of a \textit{constructive $\tau$-abstraction} where the mapping $\tau$ only groups the low-level variables into high-level (cluster) variables.} Other related works include chain graphs \citep{lauritzen:ric02} and ancestral causal graphs \citep{zhang:08} developed  to represent collections of causal diagrams equivalent under  certain properties. By contrast, our work proposes a new graphical representation of a class of compatible causal diagrams, representing limited causal knowledge when the full structural causal model is unknown.

Causal discovery algorithms %from observational data 
can be an alternative for when prior knowledge is insufficient to fully delineate a causal diagram \citep{pearl:2k, spirtes:etal00,PetersJanzingSchoelkopf17}. %\cite{zhang:08}.
%There are extensive literature on learning causal graphs from observational data. 
%\xst{However, causal structure learning remains an open, challenging problem in high-dimensional settings, particularly when unobserved/hidden variables are allowed, as is the case considered in this work.} %\xst{which is the setting we are considering (dashed bidirected edges in the causal diagram represent unobserved confounders)}. 
However, in general, it is impossible to fully recover the causal diagram based solely on observational data, without making strong assumptions about the underlying causal model, including causal sufficiency (all variables have been measured), the form of the functions (e.g., linearity, additive noise), and the distributions of the error terms (e.g. Gaussian, non-Gaussian, etc) \citep{glymour2019review}. Then, there are cases where a meaningful causal diagram cannot be learned and prior knowledge is necessary for its construction. Our work focuses on establishing a language and corresponding machinery to encode partial knowledge and infer causal effects over clusters, alleviating some challenges in causal modeling in high-dimensional settings.

 

==> R-77-CDAGS - AAAI-2023/sections/02_preliminaries.tex <==
\section{Preliminaries}
% SCM
% Causal diagram definition
% Causal diagram and kinship nomenclature

%We introduce in this section the necessary concepts and notation used throughout the paper.

\textbf{Notation.} A single variable is denoted by a (non-boldface) uppercase letter $X$ and its realized value by a small letter $x$. 
A boldfaced uppercase letter $\*X$ denotes a set (or a cluster) of variables. We use kinship relations, defined along the full edges in the graph, ignoring bidirected edges. We denote by $Pa(\*X)_G$, $An(\*X)_G$, and $De(\*X)_G$, the sets of %union of $\*X$ with its 
parents, ancestors, and descendants in $G$, respectively. A vertex $V$ is said to be \emph{active} on a path relative to
%a set 
$\*Z$ if 1) $V$ is a collider and $V$ or any of its descendants are in $\*Z$ or 2) $V$ is a non-collider and is not in $\*Z$. A path $p$ is said to be \emph{active} given (or conditioned on) $\*Z$ if every vertex on $p$ is active relative to $\*Z$. Otherwise, $p$ is said to be \emph{inactive}. Given a graph $G$, $\*X$ and $\*Y$ are d-separated by $\*Z$ if every path between $\*X$ and $\*Y$ is inactive given $\*Z$. We denote this d-separation by $(\*X \indep \*Y \mid \*Z)_{G}$. 
The mutilated graph $G_{\overline{\*X}\underline{\*Z}}$ is the result of
removing from $G$ edges %\xst{coming into} 
with an arrowhead into $\*X$ (e.g., $A \rightarrow \*X$, $A \leftrightarrow \*X$), %\xst{variables in $\*X$} 
and edges with a tail from 
%\xst{going out of variables in}
$\*Z$ (e.g., $A \leftarrow \*Z$).

%$G_\*C$ denotes the subgraph of $G$ over $\*C$.

%For $\*X, \*Y,\*Z$, we denote the conditional independence of $\*X$ and $\*Y$ conditioned on $\*Z$ by $\*X \indep \*Y \mid \*Z$. 
%we denote the d-separation between $\*X$ and $\*Y$ given $\*Z$ by $(\*X \indep \*Y \mid \*Z)_{G}$. \xadd{We call a path $p$ \emph{inactive} if and only if $(\*X \indep \*Y \mid \*Z)_{G}$ and 1) $p$ contains a chain of nodes $A  \rightarrow B \rightarrow C$ or a fork $A \leftarrow B \rightarrow C$ such that $B \in \*Z$ or 2) $p$ contains a collider $A \rightarrow B \leftarrow C$ such that $(B \cup De(B)) \cap \*Z = \emptyset$}. Otherwise, we call the path $p$ active.
% Jin
%\hl{Jin: need to review key concepts under d-separation, e.g. active/inactive path. Done!}

\textbf{Structural Causal Models (SCMs)}
%We use the language of Structural Causal Models (SCMs) \citep[pp.~204-207]{pearl:2k} as our semantical framework. % to represent causal systems.
Formally, an SCM $\mathcal{M}$ is a 4-tuple $\langle \*U, \*V, \mathcal{F}, P(\*U)\rangle$, where $\*{U}$ is a set of exogenous (latent) variables and $\*{V}$ is a set of endogenous (measured) variables. $\mathcal{F}$ is a collection of functions $\{f_i\}_{i=1}^{|\*{V}|}$ such that each endogenous variable $V_i\in\*{V}$ is %determined by 
a function $f_i\in\mathcal{F}$ %, where $f_i$ is a mapping from the respective domain 
of $\*{U}_i\cup Pa(V_i)$, % to $V_i$,
where $\*{U}_i\subseteq\*{U}$ and $Pa(V_i)\subseteq\*{V}\setminus V_i$. The uncertainty is encoded through a probability distribution over the exogenous variables, $P(\*{U})$.
Each SCM $\mathcal{M}$ induces a directed acyclic graph (DAG) with bidirected edges -- or an acyclic directed mixed graph (ADMG) -- $G(\*V, \*E)$, known as a \emph{causal diagram}, that encodes the structural relations among $\*{V}\cup\*{U}$, where every $V_i \in \*V$ is a vertex, there is a directed edge $(V_j \rightarrow V_i)$ for every $V_i \in \*V$ and $V_j \in Pa(V_i)$, and there is a dashed bidirected edge $(V_j \dashleftarrow \!\!\!\!\!\!\!\!\! \dashrightarrow V_i)$ for every pair $V_i, V_j \in \*V$ such that $\*U_i \cap \*U_j \neq \emptyset$ ($V_i$ and $V_j$ have a common exogenous parent). % We constrain our results to causal systems that are acyclic. 
%Following standard practice, we omit the exogenous variables in the causal diagrams. 
%Within the structural semantics, 
Performing an intervention $\*{X}\!\!=\!\! \*{x}$ is represented through the do-operator, \textit{do}($\*{X}\!=\!\*{x}$), which represents the operation of fixing a set $\*X$ to a constant $\*{x}$, and % regardless of their original mechanisms. Such an intervention 
induces a submodel $\mathcal{M}_\*{x}$, which is $\mathcal{M}$ with $f_X$ replaced to $x$ for every $X \in \*X$. The post-interventional distribution induced by $\mathcal{M}_\*{x}$ is denoted by $P(\*v \setminus \*x |do(\*x))$.\\ %or simply $P_\*x(\*v)$. %For further details, we refer readers to \citep{pearl:2k}.
For any subset $\*Y \subseteq \*V$, the \emph{potential response} $\*Y_{\*x}(\*u)$ is defined as the solution of $\*Y$ in the submodel $M_{\*x}$ given $\*U = \*u$. %Drawing values of exogenous variables $\*U$ following the distribution 
$P(\*U)$ then induces a \emph{counterfactual variable} $\*Y_{\*x}$.

\textbf{Pearl's Causal Hierarchy (PCH) / The Ladder of Causation } \citep{pearl:mackenzie2018, bar:etal2020} is a formal framework that divides inferential tasks into three different layers, namely, 1) associational, 2) interventional, and 3) counterfactual (see Table\ref{pearl:hierarchy}). %shows the typical activity, model and question in each layer. Any association or predictive analysis is placed in the first layer of the PCH. Effects of interventions are placed on the second layer, while counterfactuals are placed on the third layer. 
An important result formalized under the rubric of the Causal Hierarchy Theorem (CHT) \citep[Thm. 1]{bar:etal2020} states that inferences at any layer of the PCH almost never can be obtained by using solely information from lower layers.

\begin{table}[t]
{  \scriptsize
  \centering
  \begin{tabular}{@{}p{0.3cm}p{1.5cm}p{0.9cm}p{0.9cm}p{3.1cm}@{}} \hline %\toprule
   & \textbf{Level \newline (Symbol)}  &\textbf{Typical\newline Activity} & \textbf{Typical Model} & \textbf{Typical\newline Question}   \\ \hline %\midrule
   $\mathcal{L}_1$ & Associational \newline $P(y|x)$ & Seeing  & BN & What is? \newline How would seeing $X$ change my belief in $Y$?  \\ \midrule
   $\mathcal{L}_2$ & Interventional \newline $P(y|do(x),c)$ & Doing & CBN & What if? \newline What if I do $X$?  \\ \midrule
   $\mathcal{L}_3$ & Counterfactual \newline $P(y_x|x',y')$ & Imagining & SCM & Why?  \newline  What if I had acted differently?   \\ \hline %\bottomrule
  \end{tabular}}
  \caption{The Ladder of Causation / Pearl's Causal Hierarchy %Pearl's Ladder of Causation
  %\citep{pearl2018book,bar:etal2020}.
  }
  \label{pearl:hierarchy}
  \vspace{-1\intextsep}	
\end{table}

%\hl{Jin: I'd prefer using ``edge'' instead of ``arrow'' because it's natural (to me) to interpret ``an arrow'' as $\rightarrow$ but the paper is currently using ``an arrow'' to denote both $\rightarrow$ and $\leftrightarrow$. Adele: We are using edges instead of arrows now.}

% \begin{definition}[Structural Causal Model (SCM)]
% \label{def:scm} 
% A structural causal model $\mathcal{M}$ is a 4-tuple $\langle \*U, \*V, \mathcal{F}, P(\*U)\rangle$, where
% \begin{itemize}
%     \item $\*U$ is a set of background variables, also called exogenous variables, that are determined by factors outside the model;
%      \item $\*V$ is a set $\{V_1, V_2, \ldots, V_n\}$ of variables, called endogenous, that are determined by other variables in the model -- that is, variables in $\*U \cup \*V$; 
%      \item $\mathcal{F}$ is a set of functions $\{ f_1, f_2, \ldots, f_n\}$ such that each $f_i$ is a mapping from (the respective domains of) $U_{i} \cup Pa_{i}$ to $V_{i}$, where $U_{i} \subseteq \*U$, $Pa_{i} \subseteq \*V \setminus V_{i}$ is the set of endogenous parents of $V_i$, and the entire set $\mathcal{F}$ forms a mapping from $\*U$ to $\*V$. That is, for $i=1,\ldots,n$, each $f_i \in \mathcal{F}$ is such that
%     $$ v_i \leftarrow f_i(pa_{i}, u_i),$$
%     i.e., it assigns a value to $V_i$ that depends on (the values of) a select set of variables in $\*U \cup \*V$; %and 
%     \item $P(\*U)$ is a probability function defined over the domain of $\*U$. 
%   % \hfill $\blacksquare$
% \end{itemize}
% \end{definition}

% Each structural causal model can be seen as partitioning the variables involved in the phenomenon into sets of exogenous (unobserved) and endogenous (observed) variables, respectively, $\*U$ and $\*V$. The exogenous ones are determined ``outside'' of the model and their associated probability distribution, $P(\*U)$, represents a summary of the state of the world outside the phenomenon of interest. 

% Every SCM $M$ is associated with a causal diagram denoted $G$ represented as a directed acyclic graph where every variable in $V_i \in \*V$ is a vertex, and there exists a directed arrow from every variable in $Pa_{i}$ to $V_i$. Also, for every pair $V_i, V_j \in \*V$ such that $U_i \cap U_j \neq \emptyset$ there exists a bidirected arrow between $V_i$ and $V_j$.

% Lemmas shown by Tian and Pearl from with the soundness and completeness of the ID-algorithm follow: 
% %% must change and clarify this notation 
% \begin{lemma} Let $A \subseteq C \subseteq N.$ If $A$ is an ancestral set in $G_C$, then $\sum_{V_i \in C\backslash A} Q[C] = Q[A]$
% \end{lemma}

% \begin{lemma} Let $H \subseteq N$, and we have c-components $H_i^\prime, \ldots, H_n^\prime$ in the sub graph $G_H, H_i = H_i^\prime \cap H, 1 \leq i \leq n,$ then $Q[H] = \prod_{i = 1}^n Q[H_i]$
% \end{lemma}

==> R-77-CDAGS - AAAI-2023/sections/03_clusterDAGs.tex <==
%\section{C-DAGs for Optimally Encoding Partial Structural Causal Knowledge}
\section{C-DAGs: Definition and Properties}
\label{sec:cdags}


%\section{C-DAGs: Definition and Properties}


% SCM $\mathcal{M} = \langle \*{V}, \*{U}, \mathcal{F}, P(\*{U})\rangle$ and the corresponding causal diagram $G(\*{V}, \*{E})$. Given a partition $\*C=\{\*{C}_1, \ldots, \*{C}_k\}$ of $\*V$, we do not have knowledge about the relations within each cluster

Standard causal inference tools typically require assumptions articulated through causal diagrams. We investigate the situations where the knowledge necessary to specify the underlying causal diagram $G(\*{V}, \*{E})$ over the individual variables in $\*V$ may not be available. % but we are still interested in performing probabilistic, causal, and counterfactual inferences that are valid in $G$. 
%\xadd{We propose that variables among which the causal relationships are unknown (or uncertain) are grouped as a cluster. In this way, the set of individual variables $\*V$ will be partitioned into a set of of variables $\*{C}_1, \ldots, \*{C}_k$ and only relationships among clusters are needed to be specified. Then, we address the following technical problem: }
 In particular, we assume that variables are grouped into a set of clusters of variables $\*{C}_1, \ldots, \*{C}_k$ that form a partition of $\*V$ (note that a variable may be grouped in a cluster by itself) such that we do not have knowledge about the relationships amongst the variables inside the clusters $\*C_i$ but we have some knowledge about the relationships between variables in different groups. We are interested in performing probabilistic and causal inferences about these clusters of variables; one may consider each cluster as defining a \emph{macro-variable} and our aim is to reason about these macro-variables. 

%\subsection{Formal Statement of the Problem}

Formally, we address the following technical problem: 

%\hl{causal diagram of DAG?}
\vspace{.3em}
\textbf{Problem Statement:} Consider a causal diagram $G^*$ over $\*V$ and a set of clusters of variables $\*C = \{\*C_1, \ldots, \*C_k\}$ forming a partition of $\*V$. We aim to perform probabilistic, interventional, or counterfactual inferences about the macro-variables. Can we construct a causal diagram $G^*_{\*C}$ over the macro-variables in $\*C$ such that inferences by applying standard tools (d-separation, do-calculus, ID algorithm) on $G^*_{\*C}$ are valid \emph{in the  sense they lead to the same conclusions as inferred on $G^*$}?


%we can reason about the macro-variables by directly applying d-separation, do-calculus, ID algorithm on $G_C$? The inferences on $G_C$ must be sound in the sense that the inferences on $G_C$ will lead to the same conclusions as inferred on $G^*$. 

%We are interested in performing probabilistic and causal inferences about the macro-variables $C_1, \ldots, C_k$. Can we construct a DAG/ADMG $G_C$ over macro-variables such that we can reason about the macro-variables by directly applying d-separation, do-calculus, ID algorithm on $G_C$? The inferences on $G_C$ must be sound in the sense that the inferences on $G_C$ will lead to the same conclusions as inferred on $G^*$. 

%\subsection{C-DAGs: Definition and Properties}

To this end, 
%we formally introduce 
we propose a graphical object called \textit{cluster DAGs} (or C-DAGs) to capture our partial knowledge about the underlying causal diagram over individual variables. %\xst{, which is a coarser representation of a causal diagram:} \hl{can we say that is a coarser representation of a causal diagram at this moment?}
\begin{definition}[\textbf{Cluster DAG or C-DAG}]
\label{def:cdag}
%\hl{For inferences in Layer 1, $G$ doesn't need to be a causal diagram. Could we say that $G$ is just a DAG? Then in Layer 2 we discuss the particular case in which $G$ is a causal diagram?}
Given  %causal diagram 
 an ADMG $G(\*{V}, \*{E})$ (a DAG with bidirected edges)  and a partition $\*C=\{\*{C}_1, \ldots, \*{C}_k\}$ of $\*V$, construct a graph $G_{\*{C}}(\*{C}, \*{E}_\*{C})$ over $\*C$ with a set of edges $\*E_\*C$ defined as follows:
\begin{enumerate}
    \itemsep0em 
    \item  An edge $\*{C}_i \rightarrow \*{C}_j$ is in $\*E_\*C$ if exists some $V_i \in \*{C}_i$ and $V_j \in  \*{C}_j$ such that $V_i\in Pa(V_j)$ in $G$;
    \item  A dashed bidirected edge $\*{C}_i \dashleftarrow \!\!\!\!\!\!\!\!\! \dashrightarrow \*{C}_j$ is in $\*E_\*C$ if exists some $V_i \in \*{C}_i$ and $V_j \in \*{C}_j$ such that %there is a bidirected edge 
    $V_i \dashleftarrow \!\!\!\!\!\!\!\!\! \dashrightarrow V_j$ in $G$. %$V_i$ and $V_j$ have a common exogenous parent.
\end{enumerate}
If $G_{\*{C}}(\*{C}, \*{E}_\*{C})$ contains no cycles, then we say that $\*C$ is an \emph{admissible partition} of $\*V$. We then call $G_{\*{C}}$  a \emph{cluster DAG}, or \emph{C-DAG}, compatible with $G$. 
\end{definition} 
Throughout the paper, we will use the same symbols (e.g. $\*{C}_i$) to represent both a cluster node in a C-DAG $G_{\*{C}}$ and the set of variables contained in the cluster. %\xst{in a compatible causal diagram $G$.} 

\input{figs/3_med-example}

\textbf{Remark 1.} The definition of C-DAGs does not allow for cycles in order to utilize standard graphical modeling tools that work only in DAGs. An inadmissible partition of $\*V$ means that the partial knowledge available for constructing $G_{\*{C}}$ is not enough for drawing conclusions  using the tools developed in this paper.
%\xhl{Similarly to DAGs,} the definition of C-DAGs does not allow for cycles. A cycle resulting from a partition of variables in a C-DAG occurs because knowledge informing the correct order of variables is missing. Therefore, an accurate C-DAG cannot be created in this situation, and the partition is inadmissible. For example, consider the model shown in Fig.~\ref{fig:med-example}(a). It is critical in this case to understand the relationships among $S$ or $D$ and the remaining variables, as represented in Fig.~\ref{fig:med-example}(b) and (c), respectively. 
%If such knowledge is not available, it would not be possible to separate $S$ and $D$ in clusters $\*W$ and $\*Z$, respectively, while keeping consistency of the topological order of the clusters. In this case, the most informative C-DAG that can be constructed is the one over the partition $\{ \{X, A, B, C, D, S\}, \{Y\} \}$, where no causal effect is identifiable. The definition of C-DAGs is carefully designed to precisely represent all and only the causal diagrams compatible with the knowledge available. This is an essential property necessary to ensure the validity of any causal inference drawn from a C-DAG.

%\xst{Interestingly, a causal diagram  is a C-DAG where each variable forms its own cluster, which means that all clusters are of size one. In practice, however, the relationships among every pair of variables may not be known or it may be burdensome to explicitly define them, as is common in fields like medicine and the social sciences. However, contextual or temporal knowledge may partially inform how variables are related, such that a C-DAG can be constructed.} 


\input{figs/3_cluster_EC}

\textbf{Remark 2.} Although a C-DAG is defined in terms of an underlying graph %causal diagram %\hl{or DAG?} 
$G$, \textit{in practice, one will construct a C-DAG when complete knowledge of the graph $G$ is unavailable. }
As an example of this construction, consider %the diagram in
the model of the effect of lisinopril ($X$) on the outcome of having a stroke ($Y$) in Fig.~\ref{fig:med-example}(a). If not all the relationships specified in Fig.~\ref{fig:med-example}(a) are known, a data scientist cannot construct a full causal diagram, but may still have enough knowledge to create a C-DAG. For instance, they may have partial knowledge that the covariates occur temporally before lisinopril is prescribed, or that a stroke occurs and the suspicion that some of the pre-treatment variables are causes of $X$ and $Y$. 
Specifically, they can create the cluster $\*Z = \{A, B, C, D\}$ with all the covariates, and then construct a C-DAG with edges $\*Z \rightarrow X$ and $\*Z \rightarrow Y$. Further, the data scientist may also suspect that some of the variables in $\*Z$ are confounded with $X$ and others with $Y$, an uncertainty that is encoded in the C-DAG through the bidirected edges $\*Z \dashleftarrow \!\!\!\!\!\!\!\!\! \dashrightarrow X$ and $\*Z \dashleftarrow \!\!\!\!\!\!\!\!\! \dashrightarrow Y$. 
With the additional knowledge that sleep quality ($S$) %is measured after the treatment is applied (i.e., post-treatment), and 
acts as a mediator between the treatment and outcome, the C-DAG in Fig.~\ref{fig:med-example}(b) can be constructed. 
Note that this C-DAG is consistent with the true underlying causal diagram in Fig.~\ref{fig:med-example}(a), but was constructed without knowing this diagram and using much less knowledge than what is encoded in it. %\xst{Partial knowledge of this sort couldn't be formally articulated and used up to this point.} 
Alternatively, if clusters $\*W = \{S, B\}$ and $\*Z = \{A, C\}$ are created, then the C-DAG shown in Fig.~\ref{fig:med-example}(c) would be constructed. Note that both (a) and (b) are considered valid C-DAGs because no cycles are created. Finally, if a clustering with $\*W = \{S, B\}$ and $\*Z = \{A, C, D\}$ is created,  this would lead to the C-DAG shown in Fig.~\ref{fig:med-example}(d), which is invalid. The reason is that a cycle $X \rightarrow \*W \rightarrow \*Z \rightarrow X$ is created due to the connections $X \rightarrow S$, $B \rightarrow C$, and $D \rightarrow X$ in the diagram (a).


%Note that if we consider partition  $\{\{X\}, \{Y\}, \*Z, \*W\}$, where $\*W = \{S, B\}$ and $\*Z = \{A, C, D\}$, this would lead to the graph shown in Fig.~\ref{fig:med-example}(d). The edge $\{X\} \rightarrow \*{W}$ is present since $S \in \*W$ is a function of (i.e., listens to)  $X$; the edge $\*W \rightarrow \*Z$ is present because $C \in \*Z$ listens to $B \in \*W$; the edge $\*Z \rightarrow X$ is present since $X$ listens to $D \in \*Z$. These edges together create a cycle, therefore $G_{\*C''}$ is not a valid C-DAG.


\textbf{Remark 3.} It is important to note that a C-DAG $G_{\*{C}}$ as defined in Def.~\ref{def:cdag} is merely a graph over clusters of nodes ${\*C_1, ..., \*C_k }$, and does not have a priori the semantics and properties  of a BN or CBN over macro-variables $\*C_i$. It's not clear, for example, whether the cluster nodes $\*C_i$ satisfy the Markov properties w.r.t. the graph $G_{\*{C}}$. Rather, a C-DAG can be seen as a graphical representation of an equivalence class (EC, for short) of graphs that share the relationships among the clusters while allowing for any possible relationships among the variables within each cluster. 
For instance, in Fig.~\ref{fig:C-EC}, the diagrams (a) and (b) can be represented by C-DAG $G_{\*{C}_1}$ (top) and can, therefore, be thought of as being members of an EC represented by $G_{\*{C}_1}$. The same can be concluded for diagrams  (c) and (d), both represented by C-DAG $G_{\*{C}_2}$. 
The graphical representation of this ECs are shown in Fig.~\ref{fig:clusterEC}, where on the left we have the space of all possible ADMGs, and on the right the space of C-DAGs. 
% we identify an effect in a C-DAG (e.g., the C-DAG $G_{\*C_1}$ in Fig.~\ref{fig:C-EC}) if it is identifiable in all compatible causal diagrams (i.e., diagrams $(a)$, $(b)$ and all other diagrams compatible with $G_{\*C_1}$).

%The semantics of a C-DAG must account for all these possible underlying models.
 %For instance, the two causal diagrams $G_1$ in Fig.~\ref{fig:C-EC}(a) and $G_2$ in (b) can be represented by the C-DAG $G_{\*{C}}$ in (c), and can therefore be thought of as being members of the equivalence class represented by $G_{\*{C}}$.


%\begin{wrapfigure}{r}{0.5\textwidth}
\begin{figure}
\centering
%\vspace{-2\intextsep}
\includegraphics[width=0.74\linewidth]{figs/clusterEC.png}
\caption{Identifying $P(y | do(x))$ in a C-DAG  means identifying such an effect for the entire equivalence class. In $G_{\*C_1}$, the effect is identifiable (blue) because it is identifiable in $G_{(a)}$, $G_{(b)}$, and all the other causal diagrams represented. In $G_{\*C_2}$, the same effect is non-identifiable (red), as the encoded partial knowledge is compatible with some causal diagrams in which the effect is not identifiable (e.g., $G_{(d)}$).}
\vspace{-1\intextsep}
\label{fig:clusterEC}
\end{figure}
%\end{wrapfigure}



Given the semantics of a C-DAG as an equivalence class of ADMGs, what valid inferences can one perform about the cluster variables given a C-DAG $G_{\*{C}}$? %Can these inferences be performed directly, without enumerating all the possible underlying ADMGs? 
What properties of C-DAGs are shared by all compatible ADMGs?

In principle, definite conclusions from C-DAGs can only be drawn  about properties shared among all EC's members. Going back to Fig.~\ref{fig:clusterEC}, we identify an effect in a C-DAG (e.g., $G_{\*C_1}$ in Fig.~\ref{fig:C-EC}) whenever this effect is identifiable in all members of the EC; e.g., causal diagrams $(a)$, $(b)$, and all other diagrams compatible with $G_{\*C_1}$.
Note that in this particular EC, all dots are marked with blue, which means that the effect is identifiable in each one of them. 
On the other hand, if there exists one diagram in the EC where the effect is not identifiable, this effect will not be identifiable in the corresponding C-DAG. For instance, the effect is not identifiable in the C-DAG $G_{\*C_2}$ due to diagram $(d)$ in Fig.~\ref{fig:C-EC}.



%\xst{Interestingly enough, it's certainly possible that the effect is identifiable in the true, underlying causal diagram, but identifiability will not be warranted if there exists another member of the EC such that this effect is not identifiable. In fact, this suggests a trade-off of expressiveness versus identifiability power. On the one hand, C-DAGs are more expressive than causal diagrams allowing just partial specification of knowledge to be articulated, while causal diagrams are more brittle, requiring full knowledge among all pairs of variables. On the other hand, the identification status of any query will be more likely to be positive in the case of causal diagrams than in C-DAGs, since they are much stricter. The modeling task requires one to find a balance between the amount of knowledge put in the model (C-DAGs) in a way such that identification may be achieved. }

Once the semantics of C-DAGs is well-understood, we turn our attention to computational issues. One naive approach to causal inference with cluster variables, e.g. identifying $Q = P(\*C_i|do(\*C_k))$, goes as follows --  first enumerate all causal diagrams compatible with $G_{\*{C}}$; then, evaluate the identifiability of $Q$ in each diagram; finally, output $P(\*C_i|do(\*C_k))$  if all the diagrams entail the same answer, otherwise output ``non-identifiable''. However, in practice, this approach is intractable in high-dimensional settings -- given a cluster $\*C_i$ of size $m$, the number of possible causal diagrams over the variables in $\*C_i$ is super-exponential in $m$. Can valid inferences be performed about cluster variables using C-DAGs directly, without going through exhaustive enumeration? What properties of C-DAGs are shared by all the compatible causal diagrams? The next sections present theoretical results to address these questions.

Finally, note that not all properties of C-DAGs are shared across all compatible diagrams. To illustrate, consider the case of \textit{backdoor paths}, i.e., paths between $X$ and $Y$ with an arrowhead into $X$, in Fig.~\ref{fig:C-EC}. 
The path $X \dashleftarrow \!\!\!\!\!\!\!\!\! \dashrightarrow \*Z \rightarrow Y$ in $G_{\*{C}_2}$ is active when not conditioning on $\*Z$. However, the corresponding backdoor paths in diagram  (c) are all inactive.
%the \textit{backdoor path} $X \leftarrow \*Z \rightarrow Y$, i.e., a path between $X$ and $Y$ with an arrowhead into $X$, is active in the C-DAG $G_{\*{C}}$ in Fig.~\ref{fig:C-EC}(c).  All such paths are active in $G_2$ in (b), but the only backdoor path, $X \leftarrow Z_1 \rightarrow Z_2 \leftarrow Z_3 \rightarrow Y$, in $G_1$ in (a) is inactive. 
Therefore, a d-connection in a C-DAG does not necessarily correspond to a d-connection in all diagrams in the EC. 


%In the next sections, we provide all theoretical results necessary to formalize the context in which a C-DAG can be understood as a CBN. Specifically, Theorem \ref{thm:markovrelative} shows that a C-DAG is a CBN over the clusters of variables, with its semantics defined in terms of the class of all possible underlying causal diagrams and corresponding SCMs. 



% TODO AR: check if this paragraphs can be elsewhere. 
%Interestingly, a causal diagram is a C-DAG where each variable forms its own cluster, which means that all clusters are of size one.  As discussed, in practice, all such relationships may be unknown or burdensome to explicitly define, as is common in fields like medicine and the social sciences.


%The criteria set forth in Def.~\ref{def:cdag} ensure that a C-DAG, $G_{\*{C}}$, 
% The next propositions show that C-DAGs %as defined Def.~\ref{def:cdag} 
% have two properties that will prove critical later on. Namely, they preserve adjacencies, and preserve directed paths in any compatible causal diagram, $G$, thus ensuring that order and ancestral relationships are preserved. These results will prove helpful in extending % standard 
% causal inference tools to C-DAGs, including d-separation and do-calculus. \footnote{Given space constraints, all  proofs are provided in Appendix.~\ref{appendix:proofs}.} 

% %Proposition \ref{prop:cdags_connections} states that any adjacency between variables is preserved in a compatible C-DAG.
% %Proposition \ref{prop:connection_directed_Gc} states that connections via directed paths are preserved, implying that order and ancestral relationships are preserved. 


% \begin{restatable}{proposition}{adjacencies}
% \label{prop:cdags_connections}
% (\textbf{Preservation of adjacencies}) Let $G_{\*{C}}(\*{C}, \*{E}_\*{C})$ be a C-DAG compatible with a causal diagram $G(\*{V}, \*{E})$. Consider distinct clusters $\*C_i, \*C_j \in \*C$. If $V_i, V_j \in \*V$ are adjacent in $G$ and belong to $\*C_i,\*C_j$ respectively, then $\*C_i$ and $\*C_j$ are adjacent in $G_{\*C}$. Further, if $\*C_i$ and $\*C_j$ are adjacent in $G_{\*C}$, then there exists $V_i\in \*C_i$ and $V_j\in \*C_j$ such that $V_i$ and $V_j$ are adjacent in $G$.
% \end{restatable}


% \begin{restatable}{proposition}{directedpaths}
% \label{prop:connection_directed_Gc}
% (\textbf{Preservation of directed paths})
% Let $G_{\*{C}}(\*{C}, \*{E}_\*{C})$ be a C-DAG compatible with a causal diagram $G(\*{V}, \*{E})$ and $\*C_i, \*C_j \in \*C$ be two distinct clusters. If two variables $V_i \in \*C_i$ and $V_j \in \*C_j$ are connected in $G$ by a directed path from $V_i$ to $V_j$, then the clusters $\*C_i$ and $\*C_j$ are connected  by a directed path from $\*C_i$ to $\*C_j$ in $G_{\*C}$. 
% \end{restatable}


%\textcolor{red}{ Proposition \ref{prop:cdags_connections} states that any  adjacency between variables is preserved in a compatible causal diagram. } \xadd{not sure about this statement. Proposition \ref{prop:cdags_connections} states that C-DAGs preserve adjacencies between variables in compatible causal diagrams? or any  adjacency between variables is preserved in a compatible C-DAG?}


%\begin{restatable}{lemma}{ancestral}
%\label{lem:cdags_ancestral}
%Let $G_{\*{C}}$ be a C-DAG over a set of clusters $\*C$ and $G$ be a causal diagram over a set of variables $\mathbf{V}$ compatible with $G_{\*{C}}$. The creation of a cluster $\*C_i \in \*C$ in $G_{\*{C}}$ preserves any ancestral relationship in $G$. Specifically, $\forall V \in \*{C}_i,  An(V)_G \subseteq  \bigcup An(\*{C}_i)_{G_{\*{C}}}$.
%\end{restatable}

%By the definition of a cluster, and as a result of Lemma \ref{lem:cdags_ancestral}, for any two distinct clusters $\*C_i$ and $\*C_j$, $\*C_i$ cannot be both an ancestor and a descendant of  $\*C_j$. The sets of ancestors and descendants of the cluster will only have the cluster itself in common.

%\begin{corollary} For any cluster $\*{C}_i \in \*{C}$ in a C-DAG, $G_{\*{C}}$, $An(\*{C}_i)_{G_{\*{C}}} \cap De(\*{C}_i)_{G_{\*{C}}} = \*{C}_i$.\end{corollary}


==> R-77-CDAGS - AAAI-2023/sections/04_layer1_dsep.tex <==
\section{C-DAGs for $\mathcal{L}_1$-Inferences}%: d-Separation}
%\section{D-Separation and do-Calculus in C-DAGs}
\label{sec:dsep}

%\hl{Move the next part to the section on Layer 1 inferences... }
%On the other hand, we show in the next section a pleasant and surprising result (Theorem \ref{thm:dsep_cdag_dag}) that d-separations in a C-DAG %as defined next in Definition \ref{def:dsepcdag} 
%do hold in all compatible causal diagrams. 
%This powerful result is indeed critical to deriving causal inference rules and algorithms that are applicable to \textit{all} the causal diagrams compatible with a given C-DAG (Theorems \ref{thm:docalc-cdags}-\ref{thm:ids}) regardless of the unknown relationships within each cluster.
%\hl{Provide a better introduction for this section explaining what are BN and that dseps implies c.i.}

In this section, we study probabilistic inference with C-DAGs - $\mathcal{L}_1$ inferences. We assume the underlying graph $G$ over $\*V$ is a Bayesian Network (BN) \emph{with no causal interpretation}.\footnote{For a more detailed discussion on the tension between layers $\mathcal{L}_1$ and $\mathcal{L}_2$, please refer to  \cite[Sec.~1.4.1]{bar:etal2020}.  } We aim to perform probabilistic inferences about macro-variables with $G_{\*C}$ that are valid in $G$ regardless of the unknown relationships within each cluster.

First, we extend d-separation \cite{pearl:88a}, a fundamental tool in probabilistic reasoning in BNs, to C-DAGs.  % In particular, we show that d-separations in a C-DAG hold in all compatible DAGs. 
As noticed earlier, a d-connecting path in a C-DAG does not necessarily imply that the corresponding paths in a compatible ADMG $G$ are connecting. Such paths can be either active or inactive. However, d-separated paths in a C-DAG correspond to only d-separated paths  in all compatible ADMGs.\footnote{In Appendix \ref{app:pathanalysis}, we investigate in detail how path analysis is extended to C-DAGs. We note that d-separation in ADMGs has also been called m-separation \citep{richardson2003admg}.}
These observations together, lead to the following definition where the symbol $\ast$ represents either an arrow head or tail: 

%D-separation \cite{pearl:88a} is a fundamental tool in probabilistic reasoning. In this section, we show a pleasant and surprising result that d-separations in a C-DAG hold in all compatible DAGs, regardless of the unknown relationships within each cluster.

%\begin{align}
%P(\*c\setminus \*x| do(\*x)) = \sum_{\*u} P(\*u) \prod_{k:\*C_k \in \*C \setminus \*X} P(\*c_k | pa_{\*C_k}, \*u'_k), \label{eq:tfactor}
%\end{align}
%where $Pa_{\*C_k}$ are the parents of the cluster $\*C_k$ in $G_\*{C}$ and $\*U'_k \subseteq  \*U$ such that, for any $i, j$, $\*U'_i \cap \*U'_j \neq \emptyset$ if and only if there is a bidirected edge ($\*C_i \dashleftarrow \!\!\!\!\!\!\!\!\! \dashrightarrow \*C_j$) between $\*C_i$ and $\*C_j$ in $G_\*{C}$. 

%First we proof the following $\mathcal{L}_1$-optimality result:

%\begin{proposition}[\textbf{$\mathcal{L}_1$-optimality of C-DAGs}]
%\label{prop:optL1}
%For any admissible partition $\mathbf{C}$ of $\mathbf{V}$,  the observational distribution $P(\mathbf{v}) = P(\mathbf{c})$ factorizes according to a C-DAG $G_\mathbf{C}$ constructed following Def.\ref{def:cdag} w.r.t. a DAG $G$. 

%\hl{Should this be highlighted as a prop.?}
%Moreover, $G_\mathbf{C}$ does not imply any conditional independence among clusters in $\*C$ that is not implied by $G$. %(i.e., no additional assumption is made at the macro level) 
%\end{proposition}


%}

%in causal inference from causal diagrams, which have been used extensively in the context of probabilistic and causal reasoning.
% when conditioning on a mediator, a common cause, a collider, and a collider descendant.

%In this section, we investigate extending these tools to the coarser representation of a C-DAG, when the underlying causal diagram is unknown. 

%Now that a C-DAG $G_{\*C}$ is formally characterized as a BN over $\*C$, we can show that $\mathcal{L}_1$ (probabilistic) inferences with $G_{\*C}$ can be performed through d-separations as defined next, where the symbol $\ast$ represents either an arrow head or tail: 
%Note that a seemingly active path in a C-DAG does not necessarily correspond to an active path in a compatible causal diagram. Consider the case of \textit{backdoor paths}, i.e., paths between $X$ and $Y$ with an arrowhead into $X$, in Fig.~\ref{fig:C-EC}. The paths $X \leftarrow \*Z \rightarrow Y$ in $G_{\*{C}_1}$ and $X \dashleftarrow \!\!\!\!\!\!\!\!\! \dashrightarrow \*Z \rightarrow Y$ in $G_{\*{C}_2}$ appear to be connecting when not conditioning on $\*Z$. However, the corresponding backdoor paths in diagrams (a) and (b) are all blocked. %Specifically, the backdoor path in (a) is already blocked, however the backdoor path does not appear to be blocked in the corresponding C-DAG of $G_{\*C_1}$. 
%This property of C-DAGs prevents us from saying that a d-connection in a C-DAG corresponds to a d-connection in all compatible causal diagrams in the equivalence class. On the other hand, we prove in Theorem \ref{thm:dsep_cdag_dag} the pleasant and surprising result that d-separations as defined in Def.~\ref{def:dsepcdag} do hold in all compatible causal diagrams. 

\begin{definition}[\textbf{d-Separation in C-DAGs}] 
\label{def:dsepcdag}
A path $p$ in a C-DAG $G_\*C$ is said to be d-separated (or blocked) by a set of clusters $\mathbf{Z} \subset \*C$ if and only if $p$ contains a triplet
\begin{enumerate}
    \itemsep0em 
    \item 
    $\*C_i\ast\!\! - \!\!\ast \*C_m  \rightarrow \*C_j$
    %$\*{X} \ast\!\! - \!\!\ast \*{Z} \rightarrow \*{Y}$ 
    such that the non-collider cluster $\*C_m$ is in $\*Z$, or 
    \item $\*C_i \ast\!\!\!\rightarrow \*C_m \leftarrow\!\!\!\ast \*C_j$ such that the collider cluster $\*C_m$ and its descendants are not in $\*Z$.
\end{enumerate}
A set of clusters $\*Z$ is said to d-separate two sets of clusters $\*X, \*Y \subset \*C$, denoted by $(\*X \indep \*Y \mid \*Z)_{G_{\*C}}$, if and only if $\*Z$ blocks every path from a cluster in $\*X$ to a cluster in $\*Y$.
\end{definition}

%As highlighted previously, %the $\mathcal{L}_1$ optimality
%Thm.~\ref{thm:cdag_bn} does not guarantee that a dependence implied by a C-DAG $G_\mathbf{C}$ is also implied by any compatible DAG $G$. In other words, 
%a d-connecting path in a C-DAG not necessarily implies that the corresponding paths in a compatible DAG are connecting. Such paths can be either active or inactive. However, it guarantees that any conditional independence implied by a C-DAG $G_\mathbf{C}$ is also implied by any compatible DAG $G$. In other words, d-separated paths in a C-DAG correspond to only d-separated paths in all compatible DAGs.\footnote{In Appendix \ref{app:pathanalysis}, we investigate in detail how path analysis is extended to C-DAGs.}

%Specifically, we show in 

We show in the following proposition that  the d-separation rules are  sound and complete in C-DAGs in the following sense: 
whenever a d-separation holds in a C-DAG, %according to these rules,
it holds for all ADMGs compatible with it; on the other hand, if a d-separation does not hold in a C-DAG, then there exists at least one ADMG compatible with it for which the same d-separation statement does not hold. 

\begin{restatable}{theorem}{dsepcdags}(\textbf{Soundness and completeness of d-separation in C-DAGs}).
\label{thm:dsep_cdag_dag}
%Consider 
In a C-DAG $G_{\*{C}}$, let $\*{X}, \*{Z}, \*{Y} \subset \*{C}$. If $\*{X}$ and $\*{Y}$ are d-separated by $\*{Z}$ in $G_{\*{C}}$, then, in any ADMG $G$ compatible with $G_{\*{C}}$,
%letting $\*{X}$, $\*{Y}$, $\*{Z}$ be the corresponding variables contained in $\*{X}, \*{Z}, \*{Y}$, then 
$\*{X}$ and $\*{Y}$ are d-separated by $\*{Z}$ in $G$, i.e., % that is, 
\begin{align}
(\*X \indep \*Y \mid \*Z)_{G_{\*C}} \implies (\*X \indep \*Y \mid \*Z)_{G}.  
\end{align} 
%$\*{X} = \bigcup \*{X_C}$ and $\*{Y} = \bigcup \*{Y_C} $ are d-separated by $\*{Z} = \bigcup \*{Z_C}$ where $\*X, \*Y, \*Z \subset \*V$ in  $G$.
If $\*{X}$ and $\*{Y}$ are not d-separated by $\*{Z}$ in $G_{\*{C}}$, then, there exists an ADMG $G$ compatible with $G_{\*{C}}$ where $\*{X}$ and $\*{Y}$ are not d-separated by $\*{Z}$ in $G$. 
\end{restatable}
Theorem \ref{thm:dsep_cdag_dag} implies that $G_\mathbf{C}$ does not imply any conditional independence  that is not implied by the underlying $G$. %(i.e., no additional assumption is made at the macro level) 

ADMGs are commonly used to represent BNs with latent variables (which may imply Verma constraints on $P(v)$ not captured by independence relationships \citep{tian:pea02testable-implications}) %. An ADMG $G$ is a BN if 
where the observational distribution $P(\*{v})$ factorizes according to the ADMG $G$ as follows
%\footnote{One subtlety is  ADMGs may imply Verma constraints on $P(v)$ not captured by independence relations \citep{tian:pea02testable-implications}.}
\begin{align}
P(\*v) = \sum_{\*u} P(\*u) \prod_{k:V_k \in \*V } P(v_k | pa_{v_k}, \*u_k),
\label{eq:g-factor}
\end{align}
where $Pa_{V_k}$ are the endogenous parents of $V_k$ in $G$ and $\*U_k \subseteq \*U$ are the latent parents of $V_k$.
%\footnote{One important subtlety is that ADMGs may imply Verma constraints on $P(v)$ not captured by independence relationships \citep{tian:pea02testable-implications}.}
 %\footnote{One important subtlety is that  d-separation itself does not automatically hold in DAGs with latent variables, or ADMGs.} 
 We show next  that the observational distribution $P(\*{v})$ factorizes according to the graphical structure of the C-DAG $G_\mathbf{C}$ as well. % can be treated as a BN with latent variables over macro-variables $\*C$.  

\begin{restatable}{theorem}{cdagsbn}(\textbf{C-DAG as BN}).
% \begin{theorem}[C-DAG as BN]
\label{thm:cdag_bn}
%If $G(\*V,\*E)$ is a BN over $\*V$, then the C-DAG $G_\mathbf{C}(\*C, \*E_{\*C})$ constructed w.r.t. $G$ as Def.~\ref{def:cdag} is a BN over $\*C$. Formally, 
%Let $G_\mathbf{C}(\*C, \*E_{\*C})$ be a C-DAG constructed w.r.t. $G(\*V,\*E)$ as Def.~\ref{def:cdag}. 
Let $G_\*{C}$  be a C-DAG compatible with an ADMG $G$. If the observational distribution $P(\*{v})$ factorizes according to $G$ by Eq.~(\ref{eq:g-factor}),  
%\begin{align}
%P(\*v) = \sum_{\*u} P(\*u) \prod_{k:V_k \in \*V } P(v_k | pa_{v_k}, \*u_k),
%\label{eq:g-factor}
%\end{align}
%where $Pa_{V_k}$ are the endogenous parents of $V_k$ in $G$ and $\*U_k \subseteq \*U$ are the latent parents of $V_k$, 
then %for any admissible partition $\mathbf{C}$ of $\mathbf{V}$, 
the observational distribution $P(\mathbf{v}) = P(\mathbf{c})$ factorizes according to $G_\mathbf{C}$, i.e.,
\begin{align}
P(\*c) = \sum_{\*u} P(\*u) \prod_{k:\*C_k \in \*C } P(\*c_k | pa_{\*C_k}, \*u'_k), \label{eq:g-factorc}
\end{align}
where $Pa_{\*C_k}$ are the parents of the cluster $\*C_k$, %in $G_\*{C}$ 
and $\*U'_k \subseteq  \*U$ such that, for any $i, j$, $\*U'_i \cap \*U'_j \neq \emptyset$ if and only if there is a bidirected edge ($\*C_i \dashleftarrow \!\!\!\!\!\!\!\!\! \dashrightarrow \*C_j$) between $\*C_i$ and $\*C_j$ in $G_\*{C}$. 

\end{restatable}
%In Eq.~(\ref{eq:g-factorc}) and ,  $\*{X}, \*{C}, \*{C}_k, Pa_{\*C_k}$ are %sets of cluster nodes in $G_\*{C}$  while in the distribution $P(.)$ statements, $\*{X}, \*{Y}, \*{Z}, \*{W}$ represent the sets of variables contained in the corresponding sets of clusters. 
Thm.~\ref{thm:cdag_bn} implies that 
if the underlying ADMG $G$ represents a BN with latent variables over $\*V$, then the C-DAG $G_\mathbf{C}$ represents a BN over micro-variables $\*C$.

==> R-77-CDAGS - AAAI-2023/sections/05_layer2_calc_id.tex <==
%The aforementioned d-separation criterion allows us to decide from a C-DAG $G_\*C$ whether two sets of clusters $\*X$ and $\*Y$ are d-separated given a third set $\*Z$ in \emph{any} compatible causal diagram $G$. This will be essential to establishing conditions for causal identifiability in C-DAGs.

\section{C-DAGs for $\mathcal{L}_2$-Inferences} %: do-Calculus and Causal Effect Identification}
\label{sec:do-calculus}

%\hl{Provide an introduction for this section explaining that causal inferences can be done from the causal diagram. This requires now a causal semantics, which will follow from the construction of $G_C$ from a causal diagram $G$}.

We study now interventional ($\mathcal{L}_2$) reasoning with C-DAGs. We assume the underlying graph $G$ over $\*V$ is a CBN. Our goal is to perform causal reasoning about macro-variables  with $G_{\*C}$ that are guaranteed to be valid in each $G$ of the underlying EC. We focus on extending to C-DAGs Pearl's celebrated \textit{do-calculus} \citep{pearl:95a} and the ID-algorithm \citep{tian:02thesis, shpitser:pea06a,huang:val06-complete}. % for identifying causal effects. 

%We aim to perform causal inferences with $G_{\*C}$. Armed with the understanding coming from the d-separation rules in C-DAGs, 
%First we proof the following $\mathcal{L}_2$-optimality result:

%\begin{proposition}[\textbf{$\mathcal{L}_2$-optimality of C-DAGs}]
%\label{prop:optL2}
%For any admissible partition $\mathbf{C}$ of $\mathbf{V}$ and any $\*X \subseteq \*C$, 
%the interventional distribution $P(\*v\setminus \*x | do(\*x)) = P(\*c\setminus \*x | do(\*x))$ factorizes according to 
%a causal C-DAG $G_\mathbf{C}$ constructed following Def.\ref{def:cdag} w.r.t. a causal diagram $G$. 
%\hl{add here truncated factorization}
%Moreover, $G_\mathbf{C}$ does not imply any causal or confounding relationship among clusters in $\*C$ that is not implied by $G$. %(i.e., no additional assumption is made at the macro level) 
%\end{proposition}

%%%%%%%%%%%%
%, known as the truncated factorization product, i.e.:%. 
% Let $G_\*{C}$ %(\*{C}, \*{E}_\*{C})$ 
%be a C-DAG compatible with a causal diagram $G$ associated with an SCM $\mathcal{M}=\langle \*U, \*V, \mathcal{F}, P(\*U)\rangle$. For any $\*X \subseteq \*C$, the following holds
% then representing the equivalence class of all compatible CBNs over the variables $\*V$.  %where a cluster with $N$ variables is treated as an $N$-dimensional random variable. 

\subsection*{Do-Calculus in C-DAGs}
\label{sec:docalc-cdags}
Do-calculus is a fundamental tool in causal inference from causal diagrams and has been used extensively for solving a variety of identification tasks.  We show that if the underlying ADMG $G$ is a CBN on which do-calculus rules hold, then do-calculus rules are valid in the corresponding C-DAG $G_C$.  
We first present a key lemma for proving the soundness of do-calculus in C-DAGs that the mutilation operations in a C-DAG to create $G_{\*C_{\underline{\*{X}}}}$ and $G_{\*C_{\overline{\*{X}}}}$ carry over to all compatible underlying ADMGs. This result is shown in the following:


\begin{restatable}{lemma}{mutilation}
\label{lem:graph_mutilation} 
%If a C-DAG $G_\*C$ is compatible with a causal diagram $G$, then, for $\*X_\*C, \*Z_\*C \in \*C$, $G_{\*{C}_{\overline{\*{X_\*C}} \underline{\*{Z_\*C}}}}$ is compatible with $G_{\overline{\*{X}}\underline{\*{Z}}}$, where $\*X = \bigcup \*X_\*C$ and $\*Z = \bigcup \*Z_\*C$.
If a C-DAG $G_\*C$ is compatible with an ADMG $G$, then, for $\*X, \*Z \subset \*C$, the mutilated C-DAG $G_{\*{C}_{\overline{\*{X}} \underline{\*{Z}}}}$ is compatible with the mutilated ADMG $G_{\overline{\*{X}}\underline{\*{Z}}}$. % where $\*X, \*Z$ are the set of variables in the corresponding set of clusters. 
\end{restatable} 


%One of the 
%A fundamental tool used in causal inference is Pearl's celebrated \textit{do-calculus} \cite{pearl:95a}. The do-calculus has been used extensively for solving a variety of causal effect identification tasks. 
 %we show next that the do-calculus rules are also sound in C-DAGs.
%Pearl's do-calculus is a fundamental causal inference tool and has been widely used for solving a variety of causal effect identification tasks. Armed with the d-separation rules in C-DAGs, we show in Theorem \ref{thm:docalc-cdags} that  the  do-calculus rules in causal diagrams carry over to the C-DAGs.
%Given these d-separation rules, we will show in Theorem \ref{thm:docalc-cdags} that we can use the existing do-calculus rules for determining causal effects in cluster causal diagrams. Possibly active paths should be considered active when trying to establish a d-separation necessary to apply the rules of do-calculus. 

The soundness of do-calculus in C-DAGs as stated next follows from %Propositions \ref{prop:cdags_connections} and \ref{prop:connection_directed_Gc},
Theorem~\ref{thm:dsep_cdag_dag} and Lemma~\ref{lem:graph_mutilation}. 
%\newpage
\begin{restatable}{theorem}{docalc}(\textbf{Do-calculus in causal C-DAGs}).
\label{thm:docalc-cdags}
Let $G_\*{C}$ %(\*{C}, \*{E}_\*{C})$ 
be a C-DAG compatible with an ADMG $G$. If $G$ is a CBN encoding interventional distributions $P(\cdot|do(\cdot))$, then  %associated with an SCM $\mathcal{M}$. %and let $P$ be the probability distribution induced by $\mathcal{M}$. 
for any disjoint subsets of clusters $\*{X}, \*{Y}, \*{Z}, \*{W} \subseteq \*{C}$, the following three rules hold: 

$$
\begin{aligned}
    &\textbf{Rule 1:} \ P(\*y|do(\*x), \*z, \*w) = P(\*y | do(\*x), \*w) \\
    & 
     \qquad \qquad \qquad
     \text{if } (\*{Y} \indep \*{Z} | \*{X}, \*{W})_{G_{\*{C}_{\overline{\*X}}}}  \\ 
\end{aligned}
$$

$$
\begin{aligned}
    & \textbf{Rule 2:} \ P(\*{y} | do(\*{x}), do(\*{z}), \*{w}) = P(\*{y} | do(\*{x}), \*{z}, \*{w}) \\
     & 
     \qquad \qquad \qquad
     \text{if } (\*{Y} \indep \*{Z} | \*{X}, \*{W})_{G_{\*{C}_{\overline{\*{X}} \underline{\*{Z}}}}} \\
    & \textbf{Rule 3:} \ P(\*y | do(\*x), do(\*z), \*w) = P(\*y | do(\*x), \*w) \\
    & 
    \qquad \qquad \qquad
    \text{if } (\*Y \perp \! \!\! \perp \*Z | \*X, \*W)_{G_{\*{C}_{\overline{\*X}\overline{\*Z(\*W)}}}}\\
\end{aligned}
$$
where $G_{\*{C}_{\overline{\*X}\underline{\*Z}}}$ is obtained from $G_{\*{C}}$ by removing the edges %incoming to $\*X$ and outgoing from $\*Z$,
into $\*X$ and out of $\*Z$,
and $\*Z(\*W)$ is the set of $\*Z$-clusters that are non-ancestors of any $\*W$-cluster in $G_{\*{C}_{\overline{\*X}}}$.
\end{restatable}
%In Theorem~\ref{thm:docalc-cdags}, $\*{X}, \*{Y}, \*{Z}, \*{W}$ represent both the sets of clusters in $G_\*{C}$ and the sets of variables contained in the corresponding sets of clusters. 

%Given the soundness and completeness of the d-separation rules in C-DAGs, 
 % based on Proposition \ref{prop:cdags_connections}.
 
%As a result of Proposition \ref{prop:cdags_connections}, any mutilation of a C-DAG, $G_{\*C}$, performed on a set of clusters $\*X_\*C \in \*C$ will reflect the mutilation of  a compatible causal diagram $G$ whenever it is performed on a set of variables $\*X = \bigcup \*X_\*C$. Specifically, the connections removed to create $G_{\*C_{\underline{\*{X_C}}}}$ and $G_{\*C_{\overline{\*{X_C}}}}$ would also be removed from any compatible causal diagram $G$ to create $G_{\underline{\*{X}}}$ and $G_{\overline{\*{X}}}$. 

% Given a C-DAG $G_\*C$ and a cluster $\*X_\*C \in \*C$, if a connection between two clusters $\*Y_C, \*Z_C \in \*C$ is severed during the creation of $G_{\*C_{\overline{\*X_\*C}}}$ or $G_{\*C_{\underline{\*X_\*C}}}$ from $G_{\*C}$, 
% then, in any compatible diagram $G$, the connection between the sets of variables $\*Y= \bigcup \*Y_\*C$ and $\*Z = \bigcup \*Z_\*C$ is also severed during the creation of $G_{{\overline{\*X}}}$ or $G_{\underline{\*X}}$ from $G$, where $\*X = \bigcup \*X_\*C$.
% The converse also holds true.


%This is illustrated in figure \ref{fig:mutilation}. Note that because the mutilated graph $G_{\overline{X_1}}$ was created by cutting only arrows into $X_1 \subset \*X$, there are connections destroyed in $G_{\*C_{\overline{\*{X}}}}$ that are not destroyed in $G_{\overline{X_1}}$. When the connections into $\{X_1, X_2\}$ are mutilated as $G_{\overline{X_1, X_2}}$, the severing is paralleled in $G_{\*C_{\overline{\*{X}}}}$, since $\*C[X_1, X_2] = \*X = \{X_1, X_2\}$. These results are stated formally in Corollary \ref{cor:graph_mutilation}. 

% %maybe is a lemma
% \input{figs/5-graph_mutilation-fig}
 
 We also show next that the do-calculus rules in C-DAGs are complete in the following sense:
%in the following sense:
%\footnote{\xcomment{EB: This seems a local version of completeness, or completeness of the rules. We usually say in the context of do-calc completeness for a certain task. Shouldn't this be contextualized? }} %Theorem \ref{thm:do-calc_completenes} shows the completeness of the do-calculus rules for C-DAGs. 
%\ref{thm:do-calc_soundness} ensures that
%whenever a rule of the do-calculus does not apply for a C-DAG, $G_{\*{C}}$, it also applies for every causal diagram $G$ compatible with $G_{\*{C}}$. Theorem 
%that whenever a rule of do-calculus does not apply for a C-DAG, $G_{\*{C}}$, there exists a causal diagram $G$ compatible with $G_{\*{C}}$ for which it also does not apply.

% Revisiting the example diagrams in Fig. ~\ref{fig:ignorabilitycluster} where we have a cluster $\*Z = \{Z_1, Z_2\}$

\begin{restatable}{theorem}{calccomplete}
\label{thm:do-calc_completenes}
(\textbf{Completeness of do-calculus}). %The rules of the do-calculus applied to C-DAGs are complete, in the sense that, 
If in a C-DAG $G_{\*{C}}$ a do-calculus rule does not apply, then there is a CBN $G$ compatible with $G_{\*{C}}$ for which it also does not apply.
\end{restatable}

\subsection*{Truncated Factorization %Product
\label{sec:truncate}}
An ADMG $G$ represents a CBN if the interventional distributions factorizes according to the graphical structure, known as the truncated factorization, i.e., for any $\*X \subseteq \*V$%. Specifically, 
\begin{align}
P(\*v\setminus \*x | do(\*x)) = \sum_{\*u} P(\*u) \!\!\! \prod_{k:V_k \in \*V \setminus \*X} \!\!\! P(v_k | pa_{v_k}, \*u_k),
\label{eq:g-tfactor}
\end{align}
where $Pa_{V_k}$ are the endogenous parents of $V_k$ in $G$ and $\*U_k \subseteq \*U$ are the latent parents of $V_k$. 

We show that the truncated factorization holds in C-DAGs as  if the  underlying ADMG is a CBN, in the following sense.
%Next theorem %\ref{thm:markovrelative} essentially 
%shows that C-DAGs can be treated as Causal Bayesian Networks (CBNs) \citep[Def.~16]{bar:etal2020} over macro-variables $\*C$

\begin{restatable}{theorem}{markovrelative}
\label{thm:markovrelative}
(\textbf{C-DAG as CBN})
Let $G_\*{C}$ %(\*{C}, \*{E}_\*{C})$ 
be a C-DAG compatible with an ADMG $G$. If $G$ satisfies the truncated factorization (\ref{eq:g-tfactor}) with respect to the interventional distributions,  
%If $G(\*V, \*E)$ is a causal diagram over $\*V$, then the C-DAG $G_\mathbf{C}(\*C, \*E_{\*C})$ constructed w.r.t. $G$ as Def.~\ref{def:cdag} is a CBN over $\*C$. Formally,
%, for any $\*X \subseteq \*V$, the interventional distribution $P(\*v\setminus \*x | do(\*x))$ factorizes according $G$, i.e.,
%\begin{align}
%P(\*v\setminus \*x | do(\*x)) = \sum_{\*u} P(\*u) \prod_{k:V_k \in \*V \setminus \*X} P(v_k | pa_{v_k}, \*u_k),\label{eq:g-tfactor}
%\end{align}
%where $Pa_{V_k}$ are the endogenous parents of $V_k$ in $G$ and $\*U_k \subseteq \*U$ are the exogenous parents of $V_k$, 
then, for any %admissible partition $\mathbf{C}$ of $\mathbf{V}$ and 
$\*X \subseteq \*C$, the interventional distribution $P(\*c\setminus \*x | do(\*x))$ factorizes according to $G_\mathbf{C}$, i.e., 
\begin{align}
P(\*c\setminus \*x| do(\*x)) = \sum_{\*u} P(\*u) \!\!\!  \prod_{k:\*C_k \in \*C \setminus \*X}\!\!\!  P(\*c_k | pa_{\*C_k}, \*u'_k), \label{eq:tfactor}
\end{align}
where $Pa_{\*C_k}$ are the parents of the cluster $\*C_k$,  %in $G_\*{C}$ 
and $\*U'_k \subseteq  \*U$ such that, for any $i, j$, $\*U'_i \cap \*U'_j \neq \emptyset$ if and only if there is a bidirected edge ($\*C_i \dashleftarrow \!\!\!\!\!\!\!\!\! \dashrightarrow \*C_j$) between $\*C_i$ and $\*C_j$ in $G_\*{C}$. 
\end{restatable}
Theorem \ref{thm:markovrelative} essentially 
shows that a C-DAG $G_\mathbf{C}$ can be treated as a CBN %\citep[Def.~16]{bar:etal2020} 
over the macro-variables $\*C$ if the underlying ADMG is a CBN.
%This powerful result is indeed critical to deriving causal inference rules and algorithms that are applicable to \textit{all} the causal diagrams compatible with a given C-DAG (Theorems \ref{thm:docalc-cdags}-\ref{thm:ids}) regardless of the unknown relationships within each cluster.

\subsection*{ID-Algorithm\label{sec:IDalg}}

Equipped with d-separation, do-calculus, and the truncated factorization in C-DAGs, causal inference algorithms developed for a variety of tasks that rely on a known causal diagram can be extended to C-DAGs \citep{bareinboim:pea16}. In this paper, we consider the problem of identifying causal effects from observational data using C-DAGs.

There exists a complete algorithm to determine whether $P(\*y | do(\*x))$ is identifiable from a causal diagram $G$ and the observational distribution $P(\*V)$ \citep{tian:02thesis, shpitser:pea06a,huang:val06-complete}. 
This algorithm, or ID-algorithm for short, is based on the truncated factorization,  %of the interventional distributions according to the graphical structure, known as the truncated factorization product, i.e.:%. Specifically, 
therefore, Theorem \ref{thm:markovrelative} allows us to prove that the ID-algorithm is sound and complete to systematically infer causal effects from the observational distribution $P(\*V)$ and partial domain knowledge encoded as a C-DAG $G_\*C$.
%\xst{that it is sound to apply the ID-algorithm in C-DAGs, by treating each cluster node as a single variable.} %, is sound and complete.


% Theorem \ref{thm:markovrelative} showed that the truncated factorization of the interventional distribution $P(\*y | do(\*x))$ holds in C-DAGs. This result along with the characterization and tools provided in the previous sections are crucial for proving that the ID-algorithm is sound and complete to systematically infer causal effects from the observational distribution $P(\*V)$ and partial domain knowledge encoded as a C-DAG $G_\*C$. %\xst{that it is sound to apply the ID-algorithm in C-DAGs, by treating each cluster node as a single variable.} %, is sound and complete.
\begin{restatable}{theorem}{idalgsoundcomplete}
\label{thm:ids}
(\textbf{Soundness and Completeness of ID-algorithm}).
The ID-algorithm is sound and complete when applied to a C-DAG $G_\*C$ for identifying causal effects of the form $P(\*y|do(\*x))$ from the observational distribution $P(\*V)$, where $\*X$ and $\*Y$ are sets of clusters in $G_\*C$ . 
\end{restatable}

The ID algorithm returns a formula for identifiable $P(\*y|do(\*x))$ that is valid in all causal diagrams compatible with the C-DAG $G_{\*C}$. The completeness result ensures that if the ID-algorithm fails to identify $P(\*y|do(\*x))$ from $G_{\*C}$, then there exists a causal diagram $G$ compatible with $G_{\*C}$ where the effect $P(\*y|do(\*x))$ is not identifiable. 
Appendix \ref{app:simulations} contains an experimental study evaluating the ability of C-DAGs to accurately assess the identifiability of  effects while requiring less domain knowledge for their construction.

%\hl{Since we are mentioning the most general algorithm for ctf id, should we say something about gID? -- lee:etal19}

%\xst{We have a valid algorithm for inferring causal effects from a combination of an observational distribution $P(\*V)$ and partial domain knowledge encoded as a C-DAG $G_\*C$.}

%\xst{Furthermore, we show in  Appendix \ref{app:calculus} (Theorem~\ref{thm:idalgcomplete}) that the ID-algorithm is not only sufficient but also necessary for identification from observational data (i.e., complete).}

%, and,  therefore, complete. % appendix \xadd{We also prove the completeness of the ID-algorithm in C-DAGs in the appendix.}

% %Given that C-DAGs are Causal Bayesian Networks, it follows from Lemmas  \ref{lem:ancestralsetGR} and \ref{lem:ccompGR} that 
% the ID-algorithm \citep{a} is sound and complete for identifying causal effects in C-DAGs. From a combination of observational distribution $P(\*V)$ and knowledge encoded as a C-DAG $G_\*C$, the ID-algorithm returns an estimand of the causal effect whenever the effect is identifiable in any causal diagrams $G$ compatible with $G_\*C$. If the ID-algorithm fails, then there exists at least one causal diagram compatible with the $G_\*C$ where the effect is not identifiable. 

% \begin{restatable}{theorem}{idalg}
% \label{lem:ccompGR}
% (\textbf{Soundness and completeness of the ID-algorithm})
% The ID-algorithm is sound and complete for the identification of causal effects when applied to C-DAGs. 
% \end{restatable}

\subsection*{Examples of Causal Identifiability in C-DAGs}

We show examples of identification in C-DAGs in practice. Besides illustrating identification of causal effects in the coarser graphical representation of a C-DAG, these examples demonstrate that clustering variables may lead to diagrams where effects are not identifiable. Therefore, care should be taken when clustering variables, to ensure not so much information is lost in a resulting C-DAG, such that identifiability is maintained when possible. 

%Note that, due to the coarsening of the diagram by clusters, it is possible an effect will be identifiable in some causal graph $G$, but will not be identifiable by the clustering yielding $G_{\*{C}}$. 
%This example along with Fig.~\ref{fig:a2_multipleXY} illustrate how any variable, whether a treatment, outcome or another variable in a graph, can be clustered with other variables. 


%By considering the clustering $\*{Z} =\{Z_1, Z_2\}$, any separation between $Z_1$ and $Z_2$ is lost. However, under the assumption of no unobserved confounders relative to $(Z_1, X)$ and $(Z_2, X)$, %as in diagrams (c) and (f), the effect of $X$ on $Y$ is identifiable regardless of the connections between $Z_1$ and $Z_2$. From the C-DAG $G_{\*C_1}$, the effect is given by $P(y| do(x)) = \sum_{\*z} P(y |x, \*z)P(\*z)$. If domain knowledge does not justify the assumption of no unobserved confounders relative to $(Z_1, X)$ or $(Z_2, X)$, then, from the C-DAG $G_{\*C_2}$ of diagrams (a), (b), (d), and (e), the effect is not identifiable. This results from the existence of the graphs compatible with $G_{\*C_2}$ (e.g. (d) and (e)), where the effect is not identifiable.
\vspace{0.3em}
\textbf{Identification in Fig.~\ref{fig:med-example}.} In diagram (a) the effect of $X$ on $Y$ is identifiable through backdoor adjustment \citep[pp.~79-80]{pearl:2k} over the set of variables $\{B, D\}$
%\xst{ because neither $B$ nor $D$ are descendants of $X$ and $\{B, D\}$ block all paths between $X$ and $Y$ with an arrow into $X$}.
In the C-DAG in Fig.~\ref{fig:med-example}(b), with cluster $\*{Z} = \{A, B, C, D\}$,  the effect of $X$ on $Y$ is identifiable through front-door adjustment \citep[p.~83]{pearl:2k} over $S$, given by $P(y | do(x)) = \sum_{s}P(s|x)\sum_{x^\prime}P(y|x^\prime, s)P(x^\prime)$.
%\xst{, since $S$ intercepts the directed path from $X$ to $Y$, there are no unblocked back-door paths from $X$ to $S$, and all back-door paths from $S$ to $Y$ are blocked by $X$}. 
Because this front-door adjustment holds for the C-DAG in Fig.~\ref{fig:med-example}(b) with which diagram (a) is compatible, this front-door adjustment identification formula is equivalent to the adjustment in the case of diagram (a) and gives the correct causal effect in any other compatible causal diagram. In the C-DAG in (c), the loss of separations from the creation of clusters $\*{Z} = \{A, B, C, D\}$ and $\*{W} = \{B, S\}$ render the effect no longer identifiable, indicating that there exists another graph compatible with (c) for which the effect cannot be identified. %Note that it is not possible to block all backdoor paths relative to $(X,Y)$, and $\*W$, a direct effect of $X$, is confounded. 

%Figure \ref{fig:med-example}(d) is one possible, equivalent, representation of figure \ref{fig:med-example}(a) with $\*{Z} = {A, C, D, G}$ defined as a cluster. In figure \ref{fig:med-example}(d), if the $\*W$ cluster is not observed, the effect is no longer identifiable as the backdoor path from $X$ to $Y$ through $\*{Z}$ cannot be blocked. This backdoor path is possibly active, so while it is possible for a causal diagram with this cluster representation to have a blocked path underlying the cluster, the path must be assumed to be active and must be blocked to guarantee identifiability.   Figure \ref{fig:med-example}(c) shows another representation of \ref{fig:med-example}(a) with $\*{Z} = {A, C, G}$ and $\{D\}$ defined as clusters. With this representation, the effect of $X$ on $Y$ is identifiable, represented by $P(Y | do(X)) = \sum_{\*{Z}, \{D\}} P(Y | X, \*{Z}, \{D\})P(\*{Z}, \{D\}$.  


% \input{figs/5_ID-ex1}

%\input{figs/5_ID-ex2}

% \textbf{Identification in Fig.~\ref{fig:frontdoorIDEx}.} In the C-DAG shown in (c), the effect of $X$ on $Y$ is identifiable using the front-door formula: $P(y | do(x)) = \sum_{\*{w}}P(\*{w}| x)\sum_{x^\prime}P(y | x^\prime, \*{w})P(x^\prime)$. This is the correct identification formula in diagrams (a) and (b), with $\*{W} = \{W_0, W_1\}$. Note that in (b), the formula could be  simplified to $P(y| do(x)) = P(y)$ using the marginal independence between $W_1$ and $X$. This information is lost during the clustering and the directed path from $X$ to $Y$ through $\*W$ in the C-DAG is considered possibly active. However, the front-door formula ultimately provides an equivalent expression to the true causal effect.  



% \textbf{Identification in Fig.~\ref{fig:ignorabilitycluster}.} 
% %Diagrams (a),(b),(c), and (f) encode different models over $X$, $Y$, $Z_1$, and $Z_2$ where the effect of $X$ on $Y$ is identifiable.
% In the C-DAG $G_{\*C_1}$, the effect of $X$ on $Y$ is identifiable by the backdoor adjustment over $\*Z = \{Z_1, Z_2\}$.  This implies that $P(y| do(x)) = \sum_{z_1,z_2} P(y |x, z_1, z_2)P(z_1, z_2)$ in all causal diagrams compatible with $G_{\*C_1}$ (e.g, diagrams (a) and (b)). 
% In the C-DAG $G_{\*C_2}$, the effect of $X$ on $Y$ is not identifiable. This implies that $P(y| do(x))$ is not identifiable in at least one causal diagram compatible with $G_{\*C_2}$. In other words, we cannot identify $P(y| do(x))$ while being oblivious to the relationships within the cluster 
% $\*Z = \{Z_1, Z_2\}$. Note that $P(y| do(x))$ is identifiable through adjustment over $\*Z$ in diagram (c), but this adjustment does not provide the correct effect in diagram (d), where it is not identifiable. 

% \input{figs/1_ignorability}

\input{figs/a2_multipleXY}

\textbf{Identification in Fig.~\ref{fig:a2_multipleXY}.} In causal diagram (a), the effect of %the joint intervention of 
$\{X_1, X_2\}$ on %both outcomes 
$\{Y_1, Y_2\}$ is identifiable by backdoor adjustment over $\{Z_1, Z_2\}$ as follows: $P(y_1, y_2|do(x_1, x_2)) = \sum_{z_1, z_2} P(y_1, y_2|x_1, x_2, z_1, z_2) P(z_1, z_2)$. Note, however, that the backdoor path cannot be blocked in the C-DAG $G_1$ (b) with clusters $\*X = \{X_1, X_2\}$, $\*Y = \{Y_1, Y_2\}$, and $\*Z = \{Z_1, Z_2\}$. In this case, the effect $P(\*y|do(\*x))$ is not identifiable. If the covariates $Z_1$ and $Z_2$ are not clustered together as shown in the C-DAG $G_{\*C_2}$ (c), the backdoor paths relative to $\*X$ and $\*Y$ can still be blocked despite the unobserved confounders between $Z_1$ and $\*X$ and between $Z_2$ and $\*Y$. So the effect $P(\*y|do(\*x))$ is identifiable by backdoor adjustment over $\{Z_1, Z_2\}$ as follows: $P(\*y|do(\*x)) = \sum_{z_1, z_2} P(\*y|\*x, z_1, z_2) P(z_1, z_2)$. If the treatments $X_1$ and $X_2$ are not clustered together as shown in the C-DAG $G_{\*C_3}$ (d), then the joint effect of $X_1$ and $X_2$ on the cluster $\*Y$ is identifiable and given by the following expression:  $P(\*y|do(x_1, x_2)) = \sum_{\*z, x'_1} P(\*y|x'_1, x_2, \*z) P(x'_1, \*z)$.




%\newpage
%\subsection{Causal Identification with Clustered Treatments and Outcomes}
%\label{app:idexample}

%In this section, we provide an additional example of identification of causal effects in C-DAGs where the treatment and outcome variables are clustered. 


\input{figs/a1_multipleXY}

%\textbf{Identification in Fig.~\ref{fig:a1_multipleXY}.} 
\textbf{Identification in Fig.~\ref{fig:a1_multipleXY}}. In the causal diagram (a), the effect of the joint intervention to 
$\{X_1, X_2\}$ on both outcomes 
$\{Y_1, Y_2\}$ is identifiable as follows: $P(y_1, y_2|do(x_1, x_2)) = P(y_1|x_1, x_2)\sum_{x'_1}P(y_2|x'_1, x_2, y_1)P(x'_1)$. By clustering the two treatments as $\*X$ and the two outcomes as $\*Y$, we lose the information that $X_2$ is not a confounded effect of $X_1$ and that $Y_1$ and $Y_2$ are not confounded. If this is the case, as in causal diagrams $G_2$ (b) and $G_3$ (c), the effect would not be identifiable. Note that the C-DAG (d), representing causal diagrams (a), (b), and (c), is the bow graph, where the effect $P(\*y|do(\*x))$ is also not identifiable. 

%\input{sections/simulations}

%Also, Appendix \ref{app:simulations} contains an experimental study illustrating the ability of C-DAGs to accurately assess the identifiability of a causal effect while requiring less domain knowledge for their construction.

==> R-77-CDAGS - AAAI-2023/sections/06_layer3_ctf.tex <==
\section{C-DAGs for $\mathcal{L}_3$-Inferences} %: Counterfactuals}
\label{sec:ctf}

%In this section, 
Now, we study counterfactual ($\mathcal{L}_3$) inferences in C-DAGs. We assume that the underlying graph $G$ over $\*V$ is induced by an SCM $\mathcal{M}$, and our goal is to perform counterfactual reasoning about macro-variables with $G_{\*C}$ that are always valid in $\mathcal{M}$ (while both $G$ and the SCM $\mathcal{M}$ are unknown).

We show that for any SCM over $\mathbf{V}$ with causal diagram $G$, there is an equivalent SCM over macro-variables $C$ that induces C-DAG $G_C$ and makes the same predictions about counterfactual distributions over the macro-variables. 


\begin{restatable}{theorem}{scmcdags}
\label{thm:ctf_cdags}
Let $G_\*{C}$ be a C-DAG compatible with an ADMG $G$. Assume $G$ is induced by an SCM $\mathcal{M}$, then 
%Let $\mathcal{M}$ be an SCM over $\mathbf{V}$ with causal diagram $G(\*V, \*E)$. For any valid C-DAG $G_{\*C}$ constructed w.r.t. $G$ as Def.~\ref{def:cdag}, 
there exists an SCM $\mathcal{M}_{\*C}$ over macro-variables $\*C$ such that its induced causal diagram is $G_{\*C}$ and, for any set of counterfactual variables $\*Y_{\*x}, \dots, \*Z_{\*w}$ where  $\*Y, \*X, \ldots, \*Z, \*W \subseteq \*C$, $P_{\mathcal{M}}(\*y_{\*x}, \ldots, \*z_{\*w}) = P_{\mathcal{M}_{\*C}}(\*y_{\*x}, \ldots, \*z_{\*w})$. %where the random variable $\*Y_\*x$ denotes the potential response of $\*Y$ to the action $do(\*X=\*x)$. 
\end{restatable}

Following this result, algorithms developed for a variety of counterfactual inference tasks that rely on a known causal diagram, such as the CTFID algorithm \citep{correa21nestedctf}, can %potentially 
be used in the context of C-DAGs. 
%For example, the CTFID algorithm \citep{correa21nestedctf} for the identification of nested counterfactuals from an arbitrary combination of observational and experimental distributions can be extended to C-DAGs.  %To prove some completeness of these result is somewhat more involved, since it requires finding one element of the EC in which the counterfactual distribution is not identifiable.  
% Formally,
% \begin{restatable}{corollary}{idstar}
% \label{cor:cifid}
% (\textbf{Soundness and Completeness of CTFID-algorithm}).
% The CTFID algorithm is sound and complete when applied to a C-DAG $G_\*C$ for identifying a counterfactual query $P(\*y_{\*x} \ldots, \*z_{\*w})$ from  an arbitrary combination of observational and experimental distributions , where $\*X$, $\*Y$, $\ldots, \*Z$, $\*W$ are sets of clusters in $G_\*C$ . 
% \end{restatable}

For example, consider the C-DAG $G_{C_1}$ in Fig. \ref{fig:C-EC}, where $X$ is a drug, $Y$ is a disease, and $\*Z$ is a cluster of factors potentially affecting $X$ and $Y$. Suppose that a patient who took the drug ($X = 1$) would like to know what his chances of being cured ($Y=1$) would have been had he not taken the drug ($X=0$). This quantity is defined by $P(Y_{X=0} =1 | X=1)$. The CTFID algorithm applied to $G_{C_1}$ will conclude that $P(Y_{X=0}=1 | X=1)$ is identifiable and given by $\sum_zP(Y=1|X=0, Z=z)P(Z=z|X=1)$. This formula is correct in all ADMGs compatible with $G_{C_1}$, regardless of the relationships within cluster $Z$.


%\textcolor{red}{
After all, we note that inferences in the lower layers assume less knowledge than the higher layers. On the one hand, some results about the lower layers are implied by  the higher layers. For instance, if $G$ is induced by an SCM, then $G$ represents a CBN and a BN, and Thm.~\ref{thm:ctf_cdags} implies that if the underlying $G$ is induced by an SCM, then  $G_{\*C}$ represents a CBN and a BN.   %Thms.~\ref{thm:markovrelative} and ~\ref{thm:cdag_bn}. 
If $G$ is a CBN, then it is necessarily a BN, therefore Thm.~\ref{thm:markovrelative} implies that if the underlying $G$ represents a CBN, then  $G_{\*C}$ represents  a BN. %Thm.~\ref{thm:cdag_bn}. 
On the other hand, if one does not want to commit to the SCM generative process, but can only ascertain that the truncated factorization holds (e.g., for $\mathcal{L}_2$), it's still possible to leverage the machinery developed without any loss of inferential power or making unnecessary assumptions about the upper layers.  

%Thm.~\ref{thm:ctf_cdags} implies that, for any $\*Y, \*X \subseteq \*C$, the potential response $\*Y_\*x$ can be equivalently computed as the solution of $\*Y$ in the submodel $\mathcal{M}_{\*x}$ or in the submodel $\mathcal{M}_{{\*C}_{\*x}}$. This allows us to construct a counterfactual C-DAG by applying to a C-DAG the \texttt{make-cg} algorithm introduced by  \citep{shpitser:pea07} and show that
%counterfactual tools such as the ID$^*$ algorithm \citep{shpitser:pea08-r336} is sound and complete for the task of identification of a counterfactual query from the observational distribution $P(\*V)$ and partial domain knowledge encoded as a C-DAG $G_\*C$. This is formalized in the next result:

%In this case, we can make use of the \texttt{make-cg} algorithm by \citep{shpitser:pea07} for the construction of a counterfactual C-DAGs given a C-DAG and a conjunction of counterfactual events. %, which extends the twin-network approach of \cite{balke:pea94a, balke:pea94b}.

%\hl{Should we introduce here the construction of a counterfactual C-DAG using make-cg, and prove the IC$^*$ for C-DAG?}

%\begin{restatable}{theorem}{idstar}
%\label{thm:ids}
%(\textbf{Soundness and Completeness of ID$^*$-algorithm}).The ID$^*$-algorithm is sound and complete when applied to a C-DAG $G_\*C$ for identifying a counterfactual query $P(\*y_{\*x} \ldots, \*z_{\*w})$ from the observational distribution $P(\*V)$, where $\*X$, $\*Y$, $\ldots, \*Z$, $\*W$ are sets of clusters in $G_\*C$ . 
%\end{restatable}

==> R-77-CDAGS - AAAI-2023/sections/CBN_CDAGs.tex <==
%\newpage 
\subsection{Characterization of C-DAGs as Causal Bayesian Networks}
\label{app:cdags_cbn}

In Section \ref{sec:cdags}, Remark 3, we noted that it does not follow directly from Def.~\ref{def:cdag} that a C-DAG $G_{\*C}$ has the semantics and properties of a causal diagram or Causal Bayesian Network (CBN) over the cluster nodes $\*C_i$, for $i = 1, \ldots, k$. Here we clarify how the results proved in this work allow us to characterize a C-DAG as a CBN over clustered variables, representing possibly multiple underlying CBNs over the original variables.

The semantics of a C-DAG is defined in terms of the class of all compatible causal diagrams and corresponding SCMs over $\*V$. In this way, a C-DAG can be seen as an equivalence class of causal diagrams sharing the relationships among the clusters while allowing for any possible relationships among the variables within each cluster. For instance, in Fig.~\ref{fig:C-EC2}, the DAGs $G_1$, $G_2$ induce different collections of interventional distributions over the set of variables $\*V$ (i.e, $\*P^1_{*}(\*v) \neq \*P^2_{*}(\*v)$). However, when considering the cluster $\*Z = \{Z_1, Z_2, Z_3\}$, both $G_1$ and $G_2$ are represented by the C-DAG $G_{\*{C}_1}$, which induces the same collection of interventional distributions over the clusters $\*C$ (i.e., $\*P^1_{*}(\*c) = \*P^2_{*}(\*c) = \*P^{\*{C}_1}_{*}(\*c)$). In this sense, $G_1$ and $G_2$ can be thought of as being members of the equivalence class represented by $G_{\*{C}_1}$. The same can be concluded for $G_3$, $G_4$, represented by $G_{\*{C}_2}$, and for $G_5$, $G_6$, represented by $G_{\*{C}_3}$.

\input{figs/3_collapsingGraphs.tex} 
In Section \ref{sec:dsep}, Theorem \ref{thm:dsep_cdag_dag}, we showed that a d-separation in a C-DAG $G_\*C$ implies the same d-separation in all compatible causal diagrams. Given this pleasant result, we can characterize a C-DAG as a graphical encoder of conditional independencies over the set of clusters $\*C$, but this is still insufficient to give the causal interpretation necessary for the application of causal inferences tools. In fact, the same set of conditional independencies can be encoded by different DAGs, where vertices are not necessarily arranged following a causal order. This means that different DAGs can induce the same observational distribution, while differing with respect to the induced collection of interventional distributions. For example, in Fig.~\ref{fig:C-EC2}, for DAGs $G_i$, with $i = 1, 3, 5$, it holds that $P^i(\*v) = P(\*v)$, even though $P^i(\*v|do(\*x)) \neq P^j(\*v|do(\*x))$ for any $i \neq j$ and some $\*X \subseteq \*V$. Now, at the cluster level, for all DAGs $G_i$, with $i = 1, \ldots, 6$, $P^i(\*c) = P(\*c)$), while only DAGs represented by the same C-DAG induce the same collection of interventional distributions over $\*C$.
%in Fig.~\ref{fig:C-EC}, for DAGs $G_i$, with $i = 1, 3, 5$, it holds that $P^i(\*v) = P(\*v)$, even though $P^i(\*v|do(\*x)) \neq P^j(\*v|do(\*x))$ for any $i \neq j$ and some $\*X \subseteq \*V$. 


To formalize a C-DAG $G_{\*C}$ as a CBN over the cluster variables $\*C_i \in \*C$, it is necessary to show that any distribution $P_{\*x}(\*v)$ resulting from the intervention $do(\*X = \*x)$, for any $\*X \subseteq \*C$, including the observational distribution $P(\*v)$, where $\*X = \emptyset$, factorizes according to the graphical structure of $G_{\*C}$. This result, proved in Theorem \ref{thm:markovrelative}, allows us to characterize a single C-DAG $G_\*{C}$ as an encoder of the space of all interventional distributions $\*P_{*}$ at the cluster level, i.e., over the clusters of variables $\*C_i \in \*C$. More formally, a C-DAG $G_\*{C}$, compatible with a causal diagram $G$, %associated with an SCM $\mathcal{M}=\langle \*U, \*V, \mathcal{F}, P(\*U)\rangle$, 
is a CBN for $\*P_{*}^\mathcal{M}(\*c)$, the collection of interventional distributions induced by $\mathcal{M}$, over the clusters $\*C$. 



%Note that, given a partition $\*C$ of $\*V$, a larger set of DAGs can induce the same observational distribution over the set of clusters $\*C$. For each cluster $\*C_i$ of size $m_i$, the number of possible internal structures is $N_i \times 2^{m_i (m_i -1)/2}$, where $N_i$ is the number of possible DAGs without bidirected edges over $m_i$ variables, given by a super-exponential recurrence formula (see  \url{http://oeis.org/A003024}). In Fig.~\ref{fig:C-EC}, for all DAGs $G_i$, with $i = 1, \ldots, 6$, $P^i(\*c) = P(\*c)$), while only DAGs represented by the same C-DAG induce the same collection of interventional distributions over $\*C$.

This characterization is crucial for the correct abstraction of the possible underlying causal models and validity of causal tools applied to causal C-DAGs. Identifying an effect $P(y | do(x))$ in a causal C-DAG  means identifying such an effect for the entire class of causal diagrams represented. In $G_{\*{C}_2}$, the identification formula $P(y | do(x)) = P(y|x)$ is valid for $G_3$ and $G_4$, as well as all other diagrams in the class. This effect is different in the causal diagrams represented by $G_{\*{C}_3}$ (e.g., $G_5$ and $G_6$) where $P(y|do(x)) = P(y)$. On the other hand, no expression can be derived for $P(y | do(x))$ from $G_{\*{C}_1}$ since the encoded partial knowledge is compatible with some causal diagram in which the effect is not identifiable such as $G_1$.

==> R-77-CDAGS - AAAI-2023/sections/conclusions.tex <==
\section{Conclusions}

Causal diagrams provide an intuitive language for specifying the necessary assumptions for causal inferences. Despite all their power and successes, the substantive knowledge required to construct a causal diagram -- i.e., the causal and confounded relationships among all pairs of variables -- is unattainable in some critical settings found across society, including in the health and social sciences. This paper introduces a new class of graphical models that allow for a more relaxed encoding of knowledge. In practice, when a researcher does not fully know the relationships among certain variables, under some mild assumptions delineated by Def.~\ref{def:cdag}, these variables can be clustered together. (A causal diagram is an extreme case of a C-DAG where each cluster has exactly one variable. )
We prove fundamental results to allow causal inferences within C-DAG's equivalence class, which translate to statements about all diagrams compatible with the encoded constraints. 
We develop the formal machinery for probabilistic, interventional, and counterfactual reasoning in C-DAGs following Pearl's  hierarchy assuming the (unknown) underlying model over individual variables are BN ($\mathcal{L}_1$), CBN ($\mathcal{L}_2$), and SCM ($\mathcal{L}_3$), respectively. 
These results are critical for enabling C-DAGs use in ways comparable to causal diagrams. We hope these new tools  will allow researchers to represent complex systems in a simplified way, allowing for more relaxed causal inferences when substantive knowledge is largely unavailable and coarse. 




